Learning to Play Against Unknown Opponents

We consider the problem of a learning agent who has to repeatedly play a general sum game against a strategic opponent who acts to maximize their own payoff by optimally responding against the learner's algorithm. The learning agent knows their own payoff function, but is uncertain about the payoff of their opponent (knowing only that it is drawn from some distribution $\mathcal{D}$). What learning algorithm should the agent run in order to maximize their own total utility, either in expectation or in the worst-case over $\mathcal{D}$? When the learning algorithm is constrained to be a no-regret algorithm, we demonstrate how to efficiently construct an optimal learning algorithm (asymptotically achieving the optimal utility) in polynomial time for both the in-expectation and worst-case problems, independent of any other assumptions. When the learning algorithm is not constrained to no-regret, we show how to construct an $\varepsilon$-optimal learning algorithm (obtaining average utility within $\varepsilon$ of the optimal utility) for both the in-expectation and worst-case problems in time polynomial in the size of the input and $1/\varepsilon$, when either the size of the game or the support of $\mathcal{D}$ is constant. Finally, for the special case of the maximin objective, where the learner wishes to maximize their minimum payoff over all possible optimizer types, we construct a learner algorithm that runs in polynomial time in each step and guarantees convergence to the optimal learner payoff. All of these results make use of recently developed machinery that converts the analysis of learning algorithms to the study of the class of corresponding geometric objects known as menus.

==> backup/approachability_backup.tex <==
\subsection{Approachability}
We have now restated our problem of computing an optimal algorithm in terms of computing an optimal menu. Thus, we can think of our optimization problem as searching over convex sets--except, crucially, these sets need to be \emph{approachable}. In this section we will introduce and define Blackwell approachability generally, and then describe the instantiation under which this framework translates to approachability for menus.


Consider a game between two players. The learner (first player) has a finite set of actions \( A \) with \( m \) elements, and uses mixed strategies \( x \in \Delta_m \), where \( \Delta_m \) is the simplex over \( A \). The optimizer (second player) has a finite set of actions \( B \) with \( n \) elements, and uses mixed strategies \( y \in \Delta_n \), where \( \Delta_n \) is the simplex over \( B \). The utility function \( u: \Delta_m \times \Delta_n \rightarrow \mathbb{R}^d \) is vector-valued, mapping pairs of mixed strategies to vectors in \( \mathbb{R}^d \).
\begin{definition}[Response-Satisfiability]
Let \( \cM \subseteq \mathbb{R}^d \) be a closed convex set, and let \( u: \Delta_m \times \Delta_n \rightarrow \mathbb{R}^d \) be a vector-valued payoff function. The set \( \cM \) is said to be \emph{response-satisfiable} with respect to \( u \) if for every mixed strategy \( x \in \Delta_m \) of the learner, there exists a mixed strategy \( y \in \Delta_n \) of the adversary such that
\[
u(x, y) \in \cM.
\]
\end{definition}

% Blackwell Approachability Theorem
\begin{theorem}[Blackwell Approachability Theorem]
Let \( \cM \subseteq \mathbb{R}^d \) be a closed convex set, and let \( u: \Delta_m \times \Delta_n \rightarrow \mathbb{R}^d \) be a vector-valued payoff function. If \( \cM \) is response-satisfiable with respect to \( u \), then there exists a learning algorithm \( \mathcal{A} \) for the learner such that, for any sequence of strategies \( y_1, y_2, \dotsc \) chosen by the adversary, the sequence of the learner's strategies \( x_1, x_2, \dotsc \) produced by \( \mathcal{A} \) satisfies
\[
\lim_{T \rightarrow \infty} d\left( \frac{1}{T} \sum_{t=1}^T u(x_t, y_t), \cM \right) = 0,
\]
where \( d\left( \mathbf{v}, \cM \right) = \inf_{\mathbf{m} \in \cM} \| \mathbf{v} - \mathbf{m} \| \) denotes the Euclidean distance from vector \( \mathbf{v} \) to the set \( \cM \).
\end{theorem}

Now, consider some set $\cS$ in $m \cdot n$-dimensional space. We would like to know if $\cS$ is a valid menu; that is, if it is the menu of some well-defined algorithm playing a repeated $m$ by $n$ game. This is equivalent to $\cS$ being approachable in the following game\footnote{Note that this definition is agnostic of the utilities of the true repeated game that $\cS$ is deployed on.}:

\begin{definition}[Menu Approachability Game, action perspective] \label{def:menu_game_a}
    The \emph{Menu Approachability Game} \( G \) has \( m \) actions for the learner, \( n \) actions for the follower, and utility vectors in \( \mathbb{R}^d \) with \( d = n \cdot m \), defined as follows:

    For each pair of actions \( (i, j) \) where \( i \in [m] \) and \( j \in [n] \), the utility vector \( u(i, j) \in \mathbb{R}^k \) is defined by:
    \[
    u(i, j) = \mathbf{e}_{(i, j)},
    \]
    where \( \mathbf{e}_{(i, j)} \) is the standard basis vector in \( \mathbb{R}^k \) with a 1 at the coordinate corresponding to the pair \( (i, j) \) and zeros elsewhere.
\end{definition}
We refer to this game as the action space game. It is also useful for us to view these sets from a different perspective: instead of bounding what move pair distributions are possible, instead they bound what utility combinations are possible over optimizer types.

\begin{definition}[Menu Approachability Game, utility perspective] \label{def:menu_game_u}
    The \emph{Menu Approachability Game} \( G \) has \( m \) actions for the learner, \( n \) actions for the follower, and utility vectors in \( \mathbb{R}^d \) with \( d = k \), defined as follows:

    For each pair of actions \( (i, j) \) where \( i \in [m] \) and \( j \in [n] \), the utility vector \( u(i,j) \in \mathbb{R}^k \) has entries defined as follows, $\forall s \in 1,\ldots k$:
    \[
    u(i, j)[s] = u_{O,s}(i,j)
    \]
    where \( u_{O,s}(i,j) \) is the utility of the $s$-th optimizer. 
\end{definition}
We refer to this game as the utility space game. The following theorems are restatements of Theorem~\ref{thm:characterization}:

\begin{theorem}[Menu Approachability, action perspective]
Let \( \cM \subseteq \mathbb{R}^k \) be a closed convex set, and let \( u: \Delta_m \times \Delta_n \rightarrow \mathbb{R}^{n \cdot m} \) be vector-valued payoff function in the utility-Menu approachability game. If \( \cM \) is response-satisfiable with respect to \( u \), then $\cM$ is a valid menu.
\end{theorem}

\begin{theorem}[Menu Approachability, utility perspective]
Let \( \cM \subseteq \mathbb{R}^k \) be a closed convex set, and let \( u: \Delta_m \times \Delta_n \rightarrow \mathbb{R}^{n \cdot m} \) be vector-valued payoff function in the payoff-Menu approachability game. If \( \cM \) is response-satisfiable with respect to \( u \), then $\cM$ is a valid menu.
\end{theorem}



We define some Euclidean set notation that features in our algorithms and proofs. 
\begin{definition}[Point-to-set Distance] For some point $x$ in $\mathbb{R}^{d}$ and some convex set $D$ in $\mathbb{R}^{d}$, let the point-to-set distance $\rho(x,D) = \inf_{y \in D}||x - y||_2$.
\end{definition}

\begin{definition}[$\epsilon$-Expansion and $\epsilon$-contraction of a Set] Consider some set $D \in \mathbb{R}^{d}$. The $\epsilon$-expansion of $D$ is the set $D^{\epsilon}$ such that
\begin{equation}
    D^{\epsilon} = \{x : \rho(x,D) \leq \epsilon \}
\end{equation}

Conversely, $D$ is the $\epsilon$-contraction of $D^{\epsilon}$.
\end{definition}



==> backup/intro_backup.tex <==
\section{Introduction}

We consider the problem of a learning agent who has to repeatedly play against a strategic agent, called the optimizer, who acts to maximize their own payoff by optimally responding against the learner's algorithm. This setting captures a wide range of problems that address applications such as ad-auctions, airport security, etc. These problems are usually posed in an asymmetric information setting, where the learner has partial or no information about the optimizer, who, on the other hand, has full knowledge of the learner's payoff function. 

A rich line of recent work~(\cite{deng2019strategizing, brown2024learning, arunachaleswaran2024paretooptimal}, etc.) explores what constitutes a good algorithmic strategy for a learner who starts the interaction knowing nothing about the optimizer, but gets to observe their behavior on each round of play. Finding a learner algorithm to maximize the learner's payoff is not a well defined problem in this setting, since the resultant dynamics depend upon the optimizer's payoff, which is information not available to the learner at the time of picking their algorithm. Consequently, the quality of the learner's algorithm must be evaluated through the satisfaction of some other properties. The canonical answer from game theory and online learning is the property of no-regret, which implies a sublinear cap on the worst case improvement of switching to the optimal strategy in-hindsight on any transcript. The works mentioned above further augment the notion of a good learning algorithm by coming up with additional properties such as non-manipulability (the optimizer has a best-response that is static over time) and pareto-optimality (no other algorithm does better against all optimizers) and demonstrating specific algorithms that satisfy these properties. At the other end of the problem spectrum, the learner has full information about the optimizer's payoff function, making this a Stackelberg equilibrium problem in algorithm space (the learner commits to an algorithm that maximizes their payoff against an optimizer that best-responds with their own algorithm). Recent work has resolved the algorithmic question of efficiently finding this optimal commitment~\cite{zuo2015optimal,collina2023efficient}.

However, little is understood about the problem setting where the learner knows a prior from which the optimizer's type/payoff is sampled at the start of the interaction. Finding the optimal commitment that maximizes the learner's expected payoff is known to be computationally hard in the one-shot version of the problem~\cite{conitzer2006computing}. Even solving the one-shot version of the problem (and using it for each round) would not necessarily translate to finding an optimal commitment in algorithm space (See~\cite{collina2023efficient} for a separation). 
Our work addresses this fundamental open problem by designing algorithms for the following settings --

\begin{itemize}
    \item We show a polynomial time construction of the optimal commitment algorithm over the space of all no-regret algorithms.
    \item For repeated games with constant sized action sets, and for repeated games where the prior has constant support size, we show a polynomial time construction of the (unconstrained) optimal commitment algorithm for the learner.
\end{itemize}

We emphasize the difficulty of the problem of searching over algorithmic commitments. In particular, there is an intricate interplay between the learner's attempts to learn the optimizer's type based on repeated interactions and the optimizer's strategizing (non-myopically) to potentially mislead any such attempts to maximize their own payoff. %We bypass these considerations by coming up with a revelation-mechanism style construction where the otpimizer is incentivized to report their true type at the start of the interaction. 
Our results are based upon a technical tool developed in~\cite{arunachaleswaran2024paretooptimal}  that replaces the analysis of learning algorithms with the analysis of convex sets called menus. Each learning algorithm is mapped to a corresponding menu, and while this mapping loses some information (for instance, different algorithms can map to the same menu), it preserves (and simplifies) our ability to evaluate the limit-average payoff of the learning algorithm against any given optimizer. For our first result, we utilize a characterization of the menus of no-regret algorithms -- specifically a result showing that the menu of any no-regret algorithm contains the menu of a no-swap-regret (NSR) algorithm and that all NSR algorithms have the same menu. This allows us to searching over all No-Regret algorithms to solving a single Linear Program to find the optimal algorithm. For the second result , we utilize a characterization of all convex sets that are realized as the menus of some learning algorithm. This characterization rewrites menus as approachable sets (in the context of Blackwell Approachability~\cite{blackwell1956analog}) of a specific vector valued game. This allows us to use an algorithm of~\cite{mannor2009approachability} that tests the approachability of a set to search for an optimal menu. We complement our second result by showing a NP-hardness barrier to converting our particular approach (of testing Blackwell approachability) into a procedure that runs in time polynomial in the number of actions as well as the number of types.

==> backup/menus_backup.tex <==
In aid of proving our main results, we adopt the framework described in~\cite{arunachaleswaran2024paretooptimal} for the analysis
of learning algorithms. In essence, this framework swaps out analyzing learning algorithms directly in favor of analyzing convex sets in $mn$ dimensional space called menus, with each algorithm having a corresponding menu.

\subsection{Menus}
\label{sec:menus}

\begin{definition}[Correlated Strategy Profile]
Each transcript $\{(x_1,y_1), (x_2, y_2) \cdots (x_t,y_t) \}$ has an associated object $\phi$, called the Correlated Strategy Profile (CSP) that is defined as 
 \[ \phi = \frac{1}{T} \sum_{t=1}^T x_t \otimes y_t \]
    
\end{definition}

All learner algorithms have associated menus, representing the possible CSPs that the optimizer can induce from some sequence of distributions. 


For an algorithm $A^{T}$ that defines the algorithm $\A$ run for $t$ rounds, define the \emph{menu} $\M(A^T) \subseteq \Delta_{mn}$ of $A^{T}$ to be the convex hull of all CSPs of the form $\frac{1}{T}\sum_{t=1}^T x_t \otimes y_t$, where $(x_1, x_2, \dots, x_T)$ is any sequence of optimizer actions and $(y_1, y_2, \dots, y_T)$ is the response of the learner to this sequence under $A^T$ (i.e., $y_t = A^{T}_t(x_1, x_2, \dots, x_{t-1})$).


If a learning algorithm $\cA$ has the property that the sequence $\M(A^1), \M(A^2), \dots$ converges under the Hausdorff metric\footnote{The \emph{Hausdorff distance} between two bounded subsets $X$ and $Y$ of Euclidean space is given by $d_H(X, Y) = \max(\sup_{x \in X} d(x, Y), \sup_{y \in Y} d(y, X))$, where $d(a, B)$ is the minimum Euclidean distance between point $a$ and the set $B$.}, we say that the algorithm $\cA$ is \emph{consistent} and call this limit value the \emph{asymptotic menu} $\M(\cA)$ of $\cA$. More generally, we will say that a subset $\M \subseteq \Delta_{mn}$ is an asymptotic menu if it is the asymptotic menu of some consistent algorithm. It is possible to construct learning algorithms that are not consistent (for example, imagine an algorithm that runs multiplicative weights when $T$ is even, and always plays action $1$ when $T$ is odd); however even in this case we can find subsequences of time horizons where this converges and define a reasonable notion of asymptotic menu for such algorithms. See the appendix of~\cite{arunachaleswaran2024paretooptimal} for a discussion of this phenomenon.


For any asymptotic menu $\M$, define $V_{L}(\M, u_O)$ to be the utility the learner ends up with under this process. Specifically, define $V_{L}(\M, u_O, \varepsilon) = \max \{ u_{L}(\csp) \mid u_O(\csp) \ge \max_{\csp \in \M} u_{O}(\csp) - \varepsilon\}$ and $V_{L}(\M, u_O) = V_{L}(\M, u_O, 0)$. We can verify that this definition is compatible with our previous definition of $V_{L}$ as a function of the learning algorithm $\cA$ (see~\cite{arunachaleswaran2024paretooptimal} for proof). 

\begin{lemma}\label{lem:menu_alg_equiv}
For any learning algorithm $\cA$, $V_{L}(\M(\cA), u_O) = V_{L}(\cA, u_O)$ and $V_{L}(\M(\cA), u_O , \varepsilon) = V_{L}^\varepsilon(\cA, u_O)$.
\end{lemma}

We refer to any point in the set $\argmax_{\csp \in \cM} \{ u_{L}(\csp) \mid u_O(\csp) \ge \max_{\csp \in \M} u_{O}(\csp) \}$ as the point picked or selected by the optimizer $u_O$ in the menu $\cM$.



%This, we can rewrite the main results of our paper in the language of menus --



\subsection{Known Results about Menus}

\begin{comment}
    

\esh{Listing the results we need below}

\begin{itemize}
    \item Menus --  Approachability
    \item Menus are upwards closed
    \item NSR menu is contained in every no-regret menu (and define no-regret and no-swap-regret menus).
\end{itemize}
\end{comment}

The first step to study menus is characterizing all convex sets that can be realized as menus by some algorithm.

\begin{theorem}[~\cite{arunachaleswaran2024paretooptimal}]\label{thm:characterization}
A closed, convex subset $\M \subseteq \Delta_{mn}$ is an asymptotic menu iff for every $x \in \Delta_{m}$, there exists a $y \in \Delta_{n}$ such that $x \otimes y \in \M$. 
\end{theorem}

An immediate corollary of this property is that menus are upwards closed by containment.
\begin{corollary}
\label{corollary:upwards_closed}
    All asymptotic menus are upwards closed, i.e. if $\cA \subseteq \cB$ and $\cA$ is a menu, then $\cB$ is also a menu.
\end{corollary}

In fact, an artifact of the proof of Theorem~\ref{thm:characterization} is that a menu with an efficient representation can be inverted via any Blackwell approachability algorithm~\cite{} and a padding argument to come up with an algorithm that asymptotically realizes the original menu.

We have defined no-regret and no-swap regret algorithms in terms of the properties of all transcripts they induce. These properties directly translate into properties of the menus that they induce.

We say that a given CSP $\csp$ is \emph{no-regret} if it satisfies the no-regret constraint

\begin{equation}\label{eq:no-regret-constraint}
\sum_{i\in[m]}\sum_{j\in[n]} \csp_{ij}u_{L}(i, j) \geq \max_{j^{*} \in [n]}\sum_{i\in[m]}\sum_{j\in[n]} \csp_{ij}u_{L}(i, j^*).
\end{equation}

\noindent
Similarly, say that the CSP $\csp$ is \emph{no-swap-regret} if, for each $j \in [n]$, it satisfies

\begin{equation}\label{eq:no-swap-regret-constraint}
\sum_{i \in [m]} \csp_{ij}u_{L}(i, j) \geq \max_{j^* \in [n]} \sum_{i \in [m]} \csp_{ij}u_{L}(i, j^*).
\end{equation}

For a fixed $u_L$, we will define the \emph{no-regret menu} $\M_{NR}$ to be the convex hull of all no-regret CSPs, and the \emph{no-swap-regret menu} $\M_{NSR}$ to be the convex hull of all no-swap-regret CSPs. The following result states that the asymptotic menu of any no-(swap-)regret algorithm is contained in the no-(swap-)regret menu.

\begin{theorem}[~\cite{arunachaleswaran2024paretooptimal}]
\label{thm:nr_nsr_containment}
If a learning algorithm $\cA$ is no-regret, then for every $u_L$, $\M(\cA) \subseteq \M_{NR}$. If $\cA$ is no-swap-regret, then for every $u_L$, $\M(\cA) \subseteq \M_{NSR}$.
\end{theorem}

Note that both $\M_{NR}$ and $\M_{NSR}$ themselves are valid asymptotic menus, since for any $x \in \Delta_{m}$, they will contain some point of the form $x \otimes y$ for some $y \in \BR_{L}(x)$. Additionally, we know an efficient representation for each menu (as a polytope with a polynomial number of constraints) as well as algorithms whose menu is exactly this set. We make critical use of the following properties (proved in~\cite{arunachaleswaran2024paretooptimal}) of all no-swap-regret algorithms and the set $\M_{NSR}$.

First, we see that all no-swap-regret algorithms have the same asymptotic menu, which is exactly the set $\M_{NSR}$.


\begin{theorem}[~\cite{arunachaleswaran2024paretooptimal}]\label{thm:unique_nsr_menu}
If $\cA$ is a no-swap-regret algorithm, then $\M(\cA) = \M_{NSR}$.
\end{theorem}



To complement this property, we see that the menu of every no-regret algorithm weakly contains  the set $\M_{NSR}$.


\begin{lemma}[~\cite{arunachaleswaran2024paretooptimal}]
\label{lem:nsr_within_all_nr}
    For any no-regret algorithm $\A$, $\M_{NSR} \subseteq \M(\A)$.
\end{lemma}


Theorem~\ref{thm:unique_nsr_menu} is significant, since we know of concise no-swap-regret algorithms (See~\cite{blum2007external},~\cite{dagan2023external},~\cite{peng2023fast}) and thus we obtain a concise algorithm which has the menu $\M_{NSR}$. Taken together with Lemma~\ref{lem:nsr_within_all_nr}, this means that we can use any No-Swap-Regret algorithm as a ``default subroutine" when constructing an optimal no-regret algorithm -- we make use of this idea in the proof of Theorem~\ref{thm:optimal_nr}.

Finally, we present an alternative view of the polytope $\M_{NSR}$, in terms of its vertices rather than its hyperplanes.

\begin{lemma}[~\cite{arunachaleswaran2024paretooptimal}]\label{lem:nsr_characterization}
The no-swap-regret menu $\M_{NSR}$ is the convex hull of all CSPs of the form $x \otimes y$, with $x \in \Delta_{m}$ and $y \in \BR_{L}(x)$.
\end{lemma}

%~\esh{Stackelberg equilibrium definition?}
\subsection{Stackelberg Equilibria}

Points of the form $x \otimes y$, with $x \in \Delta_{m}$ and $y \in \BR_{L}(x)$ have a special significance in games. They are the candidate solutions for the Stackelberg Equilibrium problem~\cite{Stack35}, which we define below.

Two players with action sets $\cB_1$ and $\cB_2$ and payoff functions $u_1$ and $u_2$ respectively play a Stackelberg game in the following manner --  player 1, who is called the leader, commits to an action $a^*$ in $\cB_1$ and player 2, called the follower, plays a best-response $BR(a^*) \in \cB_2$ that maximizes their payoff, tie-breaking in favor of the leader. The leader must pick an action $a^*$ to maximize their own resulting payoff. Formally --

\[ a^* \in \argmax_{a \in \cB_2} u_1(a,b^*) \] 

    where $b^* \in \argmax_{b \in \cB_1} u_2(a^*,b)$ and $u_1(a,b)  \ge u_1(a,b')$ for all $b' \in \argmax_{b \in \cB_2} u_2(a^*,b)$.

The resulting action pair $(a^*,b^*)$ is referred to as a Stackelberg Equilibrium of the game and the payoff of the leader is referred to as the Stackelberg Leader value.

In the normal form game version of the problem, the action sets are simplices over finite sets of base actions and the payoff functions are linear extensions over payoff matrices defined over pairs of base actions, and in these games Stackelberg Equilibria are guaranteed to exist.

\begin{theorem}[\cite{conitzer2006computing}]
\label{thm:con_stack_alg}
There exists an efficient algorithm to compute Stackelberg equilibria in normal form games.
\end{theorem}

The notion of Stackelberg equilibria allows us to reintrepret Lemma~\ref{lem:nsr_characterization} in the following manner -- the extreme points of $M_{NSR}$ are exactly the set of candidate Stackelberg equilibria defined over all possible optimizers as the leader and the learner as the follower. In other words, an asymptotic best-response for an optimizer against no-swap-regret is to play their Stackelberg leader strategy on every single round.

%\esh{Working}


\subsection{Restatement of Objective in Terms of Menus}


We restate our main problem in the language of menus. The expected payoff of a menu against a distribution of optimizers is defined as :

\begin{equation}\label{eq:menu_learner_value}
V_{L}(\M, \optdist) = \mathbb{E}_{u_O \sim \optdist} [ V_{L}(\M, u_O) ] = \sum_{i=1}^k \alpha_i V_{L}(\M, u_{O,i}) .
\end{equation}

$V_{L}^\varepsilon(\M, \optdist)$ is similarly defined mutatis mutandis. Our aim is to find a $\varepsilon$-approximate optimal menu $\M$ such that :


\[ V_{L}^\varepsilon(\cM^*, \optdist) \ge  \max_{\text{$\M$ is a valid menu}}  V_{L}(\M, \optdist) - \varepsilon\]

We can also add the additional constraint that $\M$ is no-regret, i.e. $\M \subseteq \M_{NR}$ and set $\varepsilon = 0$ to recover the problem associated with Theorem~\ref{thm:optimal_nr}. Based on this equivalence of menus and algorithms, we come up with procedures that ouptut optimal menus (Algorithms~\ref{alg:d-opt} and~\ref{alg:d-opt-2}) rather than optimal algorithmic commitments to prove Theorems~\ref{thm:optimal_nr}and~\ref{thm:main_result_without_nr_alg}. In Appendix~\ref{app:explicit_algorithms}, we show how to ``invert" these optimal menus to derive optimal algorithms.

\subsection{Generalizations of our Model}

Our results also hold for some generalized versions of these problems with minimal modification. We discuss two orthogonal generalizations below.

\begin{itemize}
    \item The optimizer's type also affects the learner's payoff. In particular, the learner now has $k$ payoff functions $\{u_{L,i}\}_{i \in [k]}$ and received payoff $u_{L,i}(a,b)$ when playing action $a$ against the optimizer type $i$'s action $b$.
    \item The objective function of interest is not the expected payoff of the learner (over draws of the optimizer), but the minimum payoff of the learner against any possible optimizer type. More generally, any objective function that is a concave function of the CSP can be maximized.
\end{itemize}

Both generalizations only entail a change in the objective functions of the linear programs (LPs) in Algorithms~\ref{alg:d-opt} and~\ref{alg:d-opt-2}. 

==> backup/modelOPT.tex <==
\section{Model and Preliminaries}


We consider a setting where two players, an \emph{optimizer} $O$ and a \emph{learner} $L$, repeatedly play a two-player bimatrix game $G$ for $T$ rounds. The game $G$ has $m$ actions for the optimizer and $n$ actions for the learner. The learner has a fixed payoff function $u_{L}: [m] \times [n] \rightarrow [-1, 1]$. However, the optimizer draws their payoff function (equivalently their type) from a  distribution $\optdist$ of support $k$ (for some finite $k$) over optimizer payoff functions at the start of the game. For some arbitrary (but consistent) ordering, let $u_{O,i} \in \mathbb{R}^{n\cdot m}$ denote the $i$th utility vector in $\optdist$ where $u_{O,i} : [m] \times [n] \rightarrow [-1, 1]$. Furthermore, let $\alpha_{i}$ denote the probability associated with utility vector $u_{O,i}$. The learner has access to this distribution over follower utilities $\optdist$ and their own utility $u_{L}$, while the follower has access to these as well as their true utility $u_{O,i} \sim \optdist$. 


\begin{definition}[Prior $\cD$] $\cD$ is a $k$-dimensional vector of tuples such that $\cD[i] = (u_{i}, p_{i})$, signifying that the optimizer has probability $p_{i}$ of having utility $u_{i}$. We also let $\cD^{u}$ refer to only the vector of utilities, and similarly we let $\cD^{p}$ refer only to the vector of probabilities. Finally, we will abuse notation and sometimes refer to the support of the distribution as $\cD$.
\end{definition}


During each round $t$, the optimizer picks a mixed strategy $x_t \in \Delta_{m}$ while the learner simultaneously picks a mixed strategy $y_{t} \in \Delta_{n}$; the learner then receives reward $u_{L}(x_t, y_t)$ and the optimizer with private type $i \in [k]$ receives reward $u_{O,i}(x_t, y_t)$ (where here we have linearly extended $u_{L}$ and $u_{O,i}$ to take domain $\Delta_{m} \times \Delta_{n}$). Both the learner and optimizer observe the full mixed strategy of the other player (the ``full-information'' setting).



The learner will employ a \emph{learning algorithm} $\cA$ to decide how to play. For our purposes, a learning algorithm is a family of horizon-dependent algorithms $\{A^T\}_{T \in \mathbb{N}}$. Each $A^{T}$ describes the algorithm the learner follows for a fixed time horizon $T$. Each horizon-dependent algorithm is a mapping from the history of play to the next round's action, denoted by a  collection of $T$ functions $A^T_1, A^T_2 \cdots A^T_T$, each of which deterministically map the transcript of play (up to the corresponding round) to a mixed strategy to be used in the next round, i.e., $A^T_t(x_1, x_2,\cdots, x_{t-1}) = y_t$. Let $\algfams$ represent the set of all learning algorithms.



We assume that the learner is able to see $u_{L}$ and $\optdist$ before committing to their algorithm $\cA$, but not the  $u_{O}$ privately drawn by the optimizer. The optimizer, who knows $u_L$ and $u_{O}$, will approximately best-respond by selecting a sequence of actions that approximately (up to sublinear $o(T)$ factors) maximizes their payoff. They break ties in the learner's favor. Formally, for each $T$ let

\begin{equation*}
    V_{O}(\cA, u_{O}, T) = \sup_{(x_1, \dots, x_T) \in \Delta_{m}^{T}} \frac{1}{T}\sum_{t=1}^{T} u_{O}(x_t, y_t)
\end{equation*}

\noindent
represent the maximum per-round utility of the optimizer with payoff $u_O$ playing against $\cA$ in a $T$ round game (here and throughout, each $y_t$ is determined by running $A^{T}_{t}$ on the prefix $x_1$ through $x_{t-1}$). For any $\eps > 0$, let 

\begin{equation*}
\cX(\cA, u_{O}, T, \eps) = \left\{(x_1, x_2, \dots, x_T) \in \Delta_{m}^T \bigm| \frac{1}{T}\sum_{t=1}^{T} u_{O}(x_t, y_t) \geq V_{O}(\cA, u_O, T) - \eps \right\}
\end{equation*}

\noindent
be the set of $\eps$-approximate best-responses for the optimizer to the algorithm $\cA$. Finally, let

\begin{equation*}
V_{L}(\cA, u_O, T, \eps) = \sup_{(x_1, \dots, x_T) \in \cX(\cA, u_O, T, \eps)} \frac{1}{T}\sum_{t=1}^{T} u_{L}(x_t, y_t)
\end{equation*}

\noindent
represent the maximum per-round utility of the learner under any of these approximate best-responses. 

We are concerned with the asymptotic per-round payoff of the learner as $T \rightarrow \infty$ and $\eps \rightarrow 0$. Specifically, let

\begin{equation}\label{eq:learner_value}
V_{L}(\cA, u_O) = \lim_{\eps \rightarrow 0} \liminf_{T \rightarrow \infty} V_{L}(\cA, u_O, T, \eps).
\end{equation}

\noindent
Note that the outer limit in \eqref{eq:learner_value} is well-defined since for each $T$, $V_{L}(A, u_O, T, \eps)$ is decreasing in $\eps$ (being a supremum over a smaller set). 

We also define an approximate measure $V^\varepsilon_L$ in the following manner -- 

\begin{equation}\label{eq:tiebreak_learner_value}
V^\varepsilon_{L}(\cA, u_O) =  \liminf_{T \rightarrow \infty} V_{L}(\cA, u_O, T, \eps).
\end{equation}


Once again, this is well defined since all payoffs are bounded in $[-1,1]$ and the lim inf always exists. This approximate measure should be understood as the optimizer best-responding approximately up to a $\varepsilon$ additive error and tie-breaking in favor of the learner.


The final objective of the learner is the expectation of the learner's asymptotic per-round payoff over the draws of the optimizer's payoff function -- 


\begin{equation}\label{eq:learner_value}
V_{L}(\cA, \optdist) = \mathbb{E}_{u_O \sim \optdist} [ V_{L}(\cA, u_O) ] = \sum_{i=1}^k \alpha_i V_{L}(\cA, u_{O,i}) .
\end{equation}

$V_L^\varepsilon(\cA,\optdist)$ is defined similarly.


{\bf Objective of the paper: } An $\varepsilon$-optimal commitment algorithm $\cA^*$ over a family of algorithms $\cF$ satisfies 

\[ V_{L}^\varepsilon(\cA^*, \optdist) \ge  \max_{\cA \in \cF}  V_{L}(\cA, \optdist) - \varepsilon\]


When $\varepsilon= 0$, we simply call the algorithm an optimal commitment algorithm over $\cF$.


Formally stated, the main results of the paper are as follows:

First, we show how to efficiently find the optimal commitment algorithm over the set of all no-regret algorithms --
\begin{theorem}
    \label{thm:optimal_nr}
    There exists an efficient algorithm (Algorithm~\ref{alg:d-opt}), i.e., polynomial time in $m,n,k$ and the number of bits used to represent each payoff,  that constructs the optimal commitment algorithm over the set $\nralgs$ of all no-regret algorithms.
\end{theorem}

Next, we show how to efficiently (polynomial time in $m,n,k$) find $\varepsilon$-optimal commitments over all algorithms for arbitrary games with a constant sized support of optimizer distributions and small games, i.e. games with constant sized action sets, with arbitrary (but finite) size distributions over optimizer payoffs.

\begin{theorem}
\label{thm:main_result_without_nr_alg}
    There exists a procedure running in time $\min \{ \text{Poly}(mn) \cdot 2^{\text{Poly}\left (k/\varepsilon \right)}, \text{Poly}(k) \cdot 2^{\text{Poly}\left (mn/\varepsilon \right)}\}$ that constructs a $\varepsilon$-optimal commitment algorithm over all possible algorithms $\algfams$.
\end{theorem}





\begin{comment}
    

\begin{definition}[Transcript]
At time $t$, the transcript of the game thus far is a $t-1$-length list of $(x,y)$ pairs, where $x$ is a distribution in $\Delta_{n}$ and $y$ is a distribution in $\Delta{m}$. 
\end{definition}

\begin{definition}[Learner Algorithm]
The learner's algorithm $\cA$ is defined as a mapping from $t$-length transcripts to actions $\in \{\Delta_{n}\}$ to play in the $t+1$th round. 
\end{definition}

We assume that given their utility the optimizer best-responds \emph{non-myopically} to the learner's algorithm with a sequence of action distributions $y_{1},...,y_{T}$, tie-breaking in favor of the learner. We write $BR_{i}(\cA)$ to denote an optimizer with utility function $u_{i}$'s best response sequence to algorithm $\cA$. Then, given some learner algorithm $\cA$, the expected utility of the learner is 

$$\sum_{i=1}^{k}u_{L}(\cA,BR_{i}(\cA)) \cdot p_{i}$$




\begin{definition}[CSP]
The CSP of a transcript is the distribution over all pure strategy action pairs, written as $\Delta_{n} \cdot \Delta_{m}$. 
\end{definition}

Note that the CSP is a sufficient statistic to compute both the learner's and the optimizer's utility, and furthermore their utilities are linear in the CSP. 

\end{comment}

==> backup/model_backup.tex <==
\section{Model and Preliminaries}


We consider a setting where two players, an \emph{optimizer} $O$ and a \emph{learner} $L$, repeatedly play a two-player bimatrix game $G$ for $T$ rounds. The game $G$ has $m$ actions for the optimizer and $n$ actions for the learner. The learner has a fixed payoff function $u_{L}: [m] \times [n] \rightarrow [-1, 1]$. However, the optimizer draws their payoff function (equivalently, their type) from a distribution $\optdist$ of support $k$ (for some finite $k$) over optimizer payoff functions at the start of the game. For some arbitrary (but consistent) ordering, let $u_{O,i} \in \mathbb{R}^{n\cdot m}$ denote the $i$th utility vector in $\optdist$ where $u_{O,i} : [m] \times [n] \rightarrow [-1, 1]$. Furthermore, let $\alpha_{i}$ denote the probability associated with utility vector $u_{O,i}$. Define $B$ to the minimum difference between any two distinct entries over all the payoff matrices $\{u_{O,i}\}_{i\in [k]}$. The learner has access to this distribution over follower utilities $\optdist$ and their own utility $u_{L}$, while the follower has access to these as well as their true utility $u_{O,i} \sim \optdist$.  




During each round $t$, the optimizer picks a mixed strategy $x_t \in \Delta_{m}$ while the learner simultaneously picks a mixed strategy $y_{t} \in \Delta_{n}$; the learner then receives reward $u_{L}(x_t, y_t)$ and the optimizer with private type $i \in [k]$ receives reward $u_{O,i}(x_t, y_t)$ (where here we have linearly extended $u_{L}$ and $u_{O,i}$ to take domain $\Delta_{m} \times \Delta_{n}$). Both the learner and optimizer observe the full mixed strategy of the other player (the ``full-information'' setting).



The learner will employ a \emph{learning algorithm} $\cA$ to decide how to play. For our purposes, a learning algorithm is a family of horizon-dependent algorithms $\{A^T\}_{T \in \mathbb{N}}$. Each $A^{T}$ describes the algorithm the learner follows for a fixed time horizon $T$. Each horizon-dependent algorithm is a mapping from the history of play to the next round's action, denoted by a  collection of $T$ functions $A^T_1, A^T_2 \cdots A^T_T$, each of which deterministically map the transcript of play (up to the corresponding round) to a mixed strategy to be used in the next round, i.e., $A^T_t(x_1, x_2,\cdots, x_{t-1}) = y_t$. Let $\algfams$ represent the set of all learning algorithms.



We assume that the learner is able to see $u_{L}$ and $\optdist$ before committing to their algorithm $\cA$, but not the  $u_{O}$ privately drawn by the optimizer. The optimizer, who knows $u_L$ and $u_{O}$, will approximately best-respond by selecting a sequence of actions that approximately (up to sublinear $o(T)$ factors) maximizes their payoff. They break ties in the learner's favor. Formally, for each $T$, let

\begin{equation*}
    V_{O}(\cA, u_{O}, T) = \sup_{(x_1, \dots, x_T) \in \Delta_{m}^{T}} \frac{1}{T}\sum_{t=1}^{T} u_{O}(x_t, y_t)
\end{equation*}

\noindent
represent the maximum per-round utility of the optimizer with payoff $u_O$ playing against $\cA$ in a $T$ round game (here and throughout, each $y_t$ is determined by running $A^{T}_{t}$ on the prefix $x_1$ through $x_{t-1}$). For any $\eps > 0$, let 

\begin{equation*}
\cX(\cA, u_{O}, T, \eps) = \left\{(x_1, x_2, \dots, x_T) \in \Delta_{m}^T \bigm| \frac{1}{T}\sum_{t=1}^{T} u_{O}(x_t, y_t) \geq V_{O}(\cA, u_O, T) - \eps \right\}
\end{equation*}

\noindent
be the set of $\eps$-approximate best-responses for the optimizer to the algorithm $\cA$. Finally, let

\begin{equation*}
V_{L}(\cA, u_O, T, \eps) = \sup_{(x_1, \dots, x_T) \in \cX(\cA, u_O, T, \eps)} \frac{1}{T}\sum_{t=1}^{T} u_{L}(x_t, y_t)
\end{equation*}

\noindent
represent the maximum per-round utility of the learner under any of these approximate best-responses. 

We are concerned with the asymptotic per-round payoff of the learner as $T \rightarrow \infty$ and $\eps \rightarrow 0$. Specifically, let

\begin{equation}\label{eq:learner_value}
V_{L}(\cA, u_O) = \lim_{\eps \rightarrow 0} \liminf_{T \rightarrow \infty} V_{L}(\cA, u_O, T, \eps).
\end{equation}

\noindent
Note that the outer limit in \eqref{eq:learner_value} is well-defined since for each $T$, $V_{L}(A, u_O, T, \eps)$ is decreasing in $\eps$ (being a supremum over a smaller set). 

We also define an approximate measure $V^\varepsilon_L$ in the following manner -- 

\begin{equation}\label{eq:tiebreak_learner_value}
V^\varepsilon_{L}(\cA, u_O) =  \liminf_{T \rightarrow \infty} V_{L}(\cA, u_O, T, \eps).
\end{equation}


Once again, this is well defined since all payoffs are bounded in $[-1,1]$ and the lim inf always exists. This approximate measure should be understood as the optimizer best-responding approximately up to a $\varepsilon$ additive error and tie-breaking in favor of the learner.


The final objective of the learner is the expectation of the learner's asymptotic per-round payoff over the draws of the optimizer's payoff function -- 


\begin{equation}\label{eq:learner_value}
V_{L}(\cA, \optdist) = \mathbb{E}_{u_O \sim \optdist} [ V_{L}(\cA, u_O) ] = \sum_{i=1}^k \alpha_i V_{L}(\cA, u_{O,i}) .
\end{equation}

$V_L^\varepsilon(\cA,\optdist)$ is defined similarly.



Before setting out the main problem statements of this paper, we discuss some relevant classes of learning algorithms.


\paragraph{Classes of learning algorithms.} We will be interested in two specific classes of learning algorithms: \emph{no-regret algorithms} and \emph{no-swap-regret algorithms}

A learning algorithm $\cA$ is a \emph{no-regret algorithm} if it is the case that, regardless of the sequence of actions $(x_1, x_2, \dots, x_T)$ taken by the optimizer, the learner's utility satisfies:

\begin{equation*}
\sum_{t=1}^{T} u_{L}(x_t, y_t) \geq \left(\max_{y^* \in [n]} \sum_{t=1}^{T} u_{L}(x_t, y^*)\right) - o(T).
\end{equation*}

Let $\nralgs$ represent the set of all no-regret algorithms.

A learning algorithm $\cA$ is a \emph{no-swap-regret algorithm} if it is the case that, regardless of the sequence of actions $(x_1, x_2, \dots, x_T)$ taken by the optimizer, the learner's utility satisfies:

\begin{equation*}
\sum_{t=1}^{T} u_{L}(x_t, y_t) \geq \max_{\pi: [n] \rightarrow [n]} \sum_{t=1}^{T} u_{L}(x_t, \pi(y_t)) - o(T).
\end{equation*}

\noindent
Here the maximum is over all swap functions $\pi: [n] \rightarrow [n]$ (extended linearly to act on elements $y_t$ of $\Delta_n$). It is a fundamental result in the theory of online learning that both no-swap-regret algorithms and no-regret algorithms exist (see \cite{cesa2006prediction}).



{\bf Objective of the paper: } An $\varepsilon$-optimal commitment algorithm $\cA^*$ over a family of algorithms $\cF$ satisfies 

\[ V_{L}^\varepsilon(\cA^*, \optdist) \ge  \max_{\cA \in \cF}  V_{L}(\cA, \optdist) - \varepsilon\]


When $\varepsilon= 0$, we simply call the algorithm an optimal commitment algorithm over $\cF$. Formally stated, the main results of the paper are as follows:

First, we show how to efficiently find the optimal commitment algorithm over the set of all no-regret algorithms. 

\begin{theorem}
    \label{thm:optimal_nr}
    There exists an efficient algorithm (Algorithm~\ref{alg:d-opt}), i.e., polynomial time in $m,n,k$ and the number of bits used to represent each payoff,  that constructs the optimal commitment algorithm over the set $\nralgs$ of all no-regret algorithms.
\end{theorem}

Next, we show how to efficiently (polynomial time in $m,n,k$) find $\varepsilon$-optimal commitments over all algorithms for arbitrary games with a constant sized support of optimizer distributions and small games, i.e. games with constant sized action sets, with arbitrary (but finite) size distributions over optimizer payoffs.

\begin{theorem}
\label{thm:main_result_without_nr_alg}
    There exists a procedure running in time $\min \{ \poly(\frac{mn}{B \varepsilon}) \cdot 2^{\poly\left (k \right)}, \poly(\frac{k}{B \varepsilon}) \cdot 2^{\poly\left (mn \right)}\}$ that constructs a $\varepsilon$-optimal commitment algorithm over all possible algorithms $\algfams$.
\end{theorem}





\begin{comment}
    

\begin{definition}[Transcript]
At time $t$, the transcript of the game thus far is a $t-1$-length list of $(x,y)$ pairs, where $x$ is a distribution in $\Delta_{n}$ and $y$ is a distribution in $\Delta{m}$. 
\end{definition}

\begin{definition}[Learner Algorithm]
The learner's algorithm $\cA$ is defined as a mapping from $t$-length transcripts to actions $\in \{\Delta_{n}\}$ to play in the $t+1$th round. 
\end{definition}

We assume that given their utility the optimizer best-responds \emph{non-myopically} to the learner's algorithm with a sequence of action distributions $y_{1},...,y_{T}$, tie-breaking in favor of the learner. We write $BR_{i}(\cA)$ to denote an optimizer with utility function $u_{i}$'s best response sequence to algorithm $\cA$. Then, given some learner algorithm $\cA$, the expected utility of the learner is 

$$\sum_{i=1}^{k}u_{L}(\cA,BR_{i}(\cA)) \cdot p_{i}$$




\begin{definition}[CSP]
The CSP of a transcript is the distribution over all pure strategy action pairs, written as $\Delta_{n} \cdot \Delta_{m}$. 
\end{definition}

Note that the CSP is a sufficient statistic to compute both the learner's and the optimizer's utility, and furthermore their utilities are linear in the CSP. 

\end{comment}

==> backup/nr_optimal_backup.tex <==


\section{Optimal No-Regret Commitment %(Proof of Theorem~\ref{thm:optimal_nr})
}

\label{sec:nr}

\begin{theorem}\label{thm:proof_of_nr_alg} Algorithm~\ref{alg:d-opt} finds the optimal no-regret menu to commit for a learner with payoff $u_L$ against a distribution $\cD$ of optimizers. This algorithm runs in time polynomial in the size of the game and the support of the distribution $\cD$. 
\end{theorem}

%The observations that we made in Section~\ref{sec:menus} reduce the problem of finding the optimal no-regret commitment to that of finding the optimal no-regret menu. 
We outline Algorithm~\ref{alg:d-opt} to prove this theorem and demonstrate its correctness below.


\begin{algorithm}
\caption{Algorithm to Find the Optimal No-Regret Commitment} 
\label{alg:d-opt}
\begin{algorithmic}[1] % Adding numbering to the steps
    \STATE \textbf{Input}: Learner utility function $u_L$
    \STATE \textbf{Input}: Distribution $\mathcal{D}$ with support $k$ over $mn$-length vectors, representing possible optimizer types/ payoffs.
        \begin{itemize}
            \item Let $U_s$ denote the $s$-th payoff function.
            \item Let $\alpha_s$ be the probability of this utility.
        \end{itemize}

    \STATE Let $X$ be a $k \times mn$ matrix, where each row represents a CSP.
    
    \STATE Define $u_L(X[s])$ as the learner's utility under the $s$-th CSP $X[s]$. This is a linear function of $X[s]$.
    
    \STATE Define $u_s(X[s])$ as the $s$-th optimizer type's utility under the CSP $X[s]$. This is also a linear function of $X[s]$.
    
    \STATE Compute the single-round Stackelberg leader values $v_s$ for each optimizer utility. Let $v_s$ denote the value for optimizer type $s$.
    
    \STATE Solve the following linear program:
    \begin{align*}
        & \max \sum_{s=1}^{k} \alpha_s \cdot u_L(X[s]) \\
        \text{s.t.} \quad & 0 \leq X[s][j] \leq 1, \quad \forall s \in [k], j \in [mn] \\
        & \sum_{j=1}^{nm} X[s][j] = 1, \quad \forall s \in [k] \tag{Each row is a distribution} \\
        & u_{O,s}(X[s]) \geq v_s, \quad \forall s \in [k] \tag{The $s$-th optimizer values $X[s]$ (weakly) above their Stackelberg leader value} \\
        & u_s(X[s]) \geq u_s(X[i]), \quad \forall s, \forall i \neq s \tag{The $s$-th optimizer weakly prefers CSP $X[s]$ over any other $X[i]$} \\
        & X[s] \in \mathcal{M}_{NR}, \quad \forall s \tag{Each $X[s]$ is a no-regret CSP for the learner}
    \end{align*}
    
    \STATE \textbf{Output}: The menu  $\cM := \text{Conv} \{\mathcal{M}_{NSR} \cup \{X[1], X[2], \ldots, X[k\}\}$  
\end{algorithmic}
\end{algorithm}

\begin{comment}
    


\begin{algorithm}
\caption{DistOpt} \label{alg:d-opt}
    \begin{algorithmic}
     \STATE {\bf Input}: A learner utility $u_{L}$.
    \STATE {\bf Input}: A distribution $\cD$ of support $k$ over $mn$-length vectors, representing possible optimizer types. Let $U_{s}$ be the $s$-th payoff function and let $\alpha_{s}$ be the probability of this utility.
    \STATE Let $X$ be a $k \times mn$ matrix where each row represents a CSP.
    \STATE Let $u_{L}(X[s])$ be the utility of the learner under the $s$-th CSP $X[s]$. This is a linear function of $X[s]$. 
    \STATE  $u_{s}(X[s])$ is the utility of the $s$-th optimizer type under the CSP $X[s]$. This is also a linear function of the CSP $X[s]$. 
    \STATE Compute the single-round Stackelberg leader values $v_s$ for each possible optimizer utility function. Let the value for optimizer type $s$ be $v_{s}$.
    \STATE Solve the following linear program: 
    \STATE \begin{align*} & \max\sum_{s=1}^{k}\alpha_{s}\cdot u_{L}(X[s]) \\
     s.t. & & 0 \leq X[s][j] \leq 1,  \forall s \in [k], j \in [mn] \\
    &&  \sum_{j=1}^{nm}X[s][j] = 1,  \forall s \in [k] \tag{Each row is a distribution}\\
    &&  u_{k}(x[k]) \geq s_{k}, \forall k \tag{The $k$th optimizer weakly prefers point $x[k]$ over their static stackelberg}\\
    &&  u_{s}(X[s]) \geq u_{s}(X[i]), \forall k, \forall i \neq k \tag{The $s$-th optimizer type weakly prefers CSP $X[s]$ over any CSP $X[i]$}\\
     && X[s] \in \M_{NR}, \forall s \tag{Every $X[s]$ is a no-regret CSP for the learner}\\
    \end{align*}
    \STATE Output the menu  $\M_{NSR} \cup \left(\cup_s X_s \right)$%, and in addition all points of the form $x[k]$ $\forall k$.
    \end{algorithmic}
\end{algorithm}


\end{comment}


%\begin{theorem}{(From Pareto-Optimal Paper)} \label{thm:nsr} All no-regret menus contain the NSR menu. \end{theorem}



%\esh{Canonical NR menus}
%\esh{editing}
First, we show that all No-Regret menus can be rewritten in a succinct canonical form, without changing the payoff of the learner.
\begin{lemma} 
%\label{lemma:nr_succinct_menu}
For any no-regret menu $\M$ such that the extreme points selected by agents of each context are $X_{1},...,X_{k}$ (i.e. $X_s \in \argmax_{\phi \in \M} u_{O,s}(\phi)$ with tie-breaking in favor of the learner), consider the set $\M'$ such that $\M' = conv(M_{NSR} \cup X_{1},...,X_{k})$. Then $\M'$ is a no-regret menu and $u_{L}(\M, \cD) = u_{L}(\cM',\cD)$, and the optimizer with utility $u_{O,s}$ weakly prefers the CSP $X_{s}$ over all other points in $\cM'$. \label{lem:decomp}
\end{lemma}
\begin{proof}
    By Lemma~\ref{lem:nsr_within_all_nr}, all no-regret menus must contain the NSR menu within them implying that $\cM_{NSR} \subseteq \cM$. We also know that  $\cM_{NSR}$ itself is a menu (Theorem~\ref{thm:unique_nsr_menu}), and since the superset of a menu is also a menu (Corollary~\ref{corollary:upwards_closed}), $\cM'$ is also a menu. Further, $\cM' \subseteq \cM \subseteq \M_{NR}$ implying that $\cM'$ is a no-regret menu. %Therefore, we can equivalently write $\cM$ as $\cM \cup \M_{NSR}$. 
    Let $\cM' = conv(\cM_{NSR} \cup X_{1},...,X_{k})$ for the extreme points of $M$ selected by optimizer types with respective payoffs $u_{O,1},...,u_{Ok}$. Now, consider any utility $u_{O,s}$. %An extreme point in the direction $u_{O,s}$ in $\cM$ is $x_{s}$. 
    As $\cM' \subseteq \cM$ and $X_{s} \in M'$, an extreme point in the direction $u_{O,s}$ in $M'$ is $X_{s}$. Therefore, for all $s$, an agent with utility $u_{O,s}$ weakly prefers $X_{s}$ over all other points in $M'$. %\nat{say something about tiebreaking} 
Since $X_s$ was the result of tie-breaking in favor of the learner in $\cM$, $X_s$  will again be win the tie-break among points in $\cM'$, a subset of $\cM$, completing this proof.
\end{proof}

This lemma allows us to recast searching for the optimal no-regret menu to searching for the best possible $k$ CSPs, which we can then add to the menu $\M_{NSR
}$.

\begin{comment}
    

\end{comment}

\subsection{Proof of Theorem~\ref{thm:proof_of_nr_alg}}


Let the menu output by Algorithm~\ref{alg:d-opt} be $\cM^{*}$, and assume for contradiction that there exists some no-regret menu $\cM'$ such that $V_{L}(\cM') > V_{L}(\cM^{*})$. By Lemma~\ref{lem:decomp}, there exists some menu $\cM''$ such that $V_{L}(\cM'') = V_{L}(\cM') > V_{L}(\cM^{*})$, where $M'' = conv(M_{NSR} \cup Y_{1},...,Y_{k})$ such that the $i$-th type optimizer picks point $Y_i$ in $\cM''$. Also, $Y_i \in \M_{NR}$ since $\cM'$ is an optimal no-regret menu. Let $\cM^* = {M}_{NSR} \cup \left( \bigcup_s X_s \right)$ be the menu output by Algorithm~\ref{alg:d-opt}, we show that $V_L(\cM^*) = V_L(\cM'')$, thus obtaining a contradiction and completing the proof of this lemma. The objective function of the LP is the expected payoff of the learner when the $i$-th optimizer type picks the point $X_i$. Thus, it suffices to show for each $i \in [k]$ that $u_{O,i}(X_i) \ge u_{O,i}(X)$, $\forall X \in \cM^*$, since that would imply that $Y_1, Y_2 \cdots Y_k$ is a feasible solution to the LP. Each $X_i$ is a CSP due to the LP constraints and $X_i \in \M_{NR}$. Further the constraints guarantee that $u_{O,i}(X_i) \ge  u_{O,i}(X_j)$ for all $i,j \in [k]$. Thus, it suffices to show that for each $i \in [k]$ that $u_{O,i}(X_i) \ge u_{O,i}(X)$, $\forall X \in \cM_{NSR}$. This is in turn achieved by showing that $\max_{X \in \M_{NSR}} u_{O,i}(X) = v_i$ where $v_i$ is the Stackelberg leader value of the optimizer in the normal form game with leader payoff $u_{O,i}$ and follower payoff $u_L$, due to the corresponding constraint in the linear program. We invoke the vertex characterization of the polytope $\M_{NSR}$ (Lemma~\ref{lem:nsr_characterization}) -- all vertices are of the form $x \otimes y$, with $x \in \Delta_{m}$ and $y \in \BR_{L}(x)$. These are exactly the candidate Staceklberg equilibria of the normal form game with the optimizer (committing to $x$) as the leader and the learner as a follower (best-responding under $u_L$ to $x$). Therefore, $\max_{X \in \M_{NSR}} u_{O,i}(X) = v_i$ completing the result. Finally we note that the algorithm only solves a linear program with polynomial number of variables and constraints in the size of the problem, showing that it is computationally efficient. The only other information that it needs are the Stackelberg values, which can be found efficiently in the size of the game, completing this proof.

%\esh{editing}%But this menu satisfies the constraints of DistOpt, and therefore we have derived a contradiction.


%Proof sketch: this LP solves for the best menu which contains the NSR menu. Since every no regret menu contains the NSR menu, this is the best menu. 






%\esh{Add a note about explicitly constructing an algorithm that induces the menu generated by the algorithm - we know how to do this as a special case, but do we know of a separation/ membership oracle for this menu - that might make things cleaner }


We conclude this section by noting that $\M_{NSR}$, while part of every no-regret menu, is not by itself the optimal no-regret menu, even when the optimizer is fixed to be a single type.

\begin{lemma}
\label{lem:nsr_not_optimal}
    There exists learner utility $u_{L}$ and a distribution over optimizer types $\mathcal{D}$ such that Algorithm~\ref{alg:d-opt} performs strictly better than a no-swap regret algorithm 
\end{lemma}





==> backup/oldstuff.tex <==

\esh{Older stuff below}
\begin{theorem} (Not our theorem): There exists a membership oracle for determining whether a convex set is a valid menu such that 
\end{theorem}

\begin{lemma} If $d + \delta_{2} \in M$, then $d \in M + \delta_{2}$
\end{lemma}
\begin{proof}

\begin{itemize}

\item If $d + \delta_{2} \in M$, then this means that the $\delta_{2}$ expansion of $M$ is approachable. 

\item Now, call the following set $S$: take every CSP in the original set associated with a utility $u_{i}$, and travel $\delta_{2}$ in the direction of agent $i$'s utility vector. This leaves us with $k$ new points. Reconstruct the maximal polytope satisfying the IC constraints using these $k$ new points (PS: We can argue that these points themselves preserve the IC constraints comparing to each other) - call this set $S$. %Now, take the convex hull of these points, and then take the convex hull of this hull and the original menu. This is $S$.

\item We show that $M + \delta_{2}$ is strictly contained within $S$. Because of this, $S$ is approachable.

\item Consider the points which define $S$. By construction, each is only $\delta_{2}$-far in euclidean distance from their respective point in the original vector. If the point which define $S$ are 


\item Issue: 
\end{itemize}
\end{proof}

\begin{definition}[$(\epsilon_{1},\epsilon_{2})$-plausible approachability] Let $\delta = \frac{\epsilon_{2} - \epsilon_{1}}{2\epsilon_{1} + 2}$, and let $C_{\delta}$ be the $\delta$-covering of $\mathbb{R}^{mnk}$ such that \textcolor{blue}{[Natalie] todo: give some explicit definition of a consistent and canonical covering here. It's just important that it is the same for any polytope.}
A polytope in $\mathbb{R}^{d}$ is $(\epsilon_{1},\epsilon_{2})$-plausibly approachable if, for all vectors $d_{i}$ in $C_{\delta}$, there does \emph{not} exist a $q \in \Delta[m]$ (the optimizer's actions) such that
\begin{equation}
    \max_{x \in D^{\epsilon_{1}}}d_{i}^{T}x < d_{i}^{T}M(a,q) \ \ \forall a \in \Delta[n]
\end{equation}
\end{definition}


\begin{lemma} If $x \cdot u_{j} \leq u_{j} \cdot v'[j], \ \ \forall j$, then it must be the case that either $x \cdot u_{j} \leq u_{j} \cdot v_{1}[j], \ \ \forall j$, or $x \cdot u_{j} \leq u_{j} \cdot v_{2}[j], \ \ \forall j$.
\end{lemma}
\begin{proof}
    Assume for contradiction that $\exists$ $j_{1}$, $j_{2}$ such that $x \cdot u_{j} > u_{j} \cdot v_{1}[j_{1}]$ and $x \cdot u_{j} > u_{j} \cdot v_{2}[j_{2}]$. Then, 
\end{proof}

\begin{lemma} $\epsilon$-plausible approachability of $P(v)$ is a convex property of $v$.
\end{lemma}

\begin{proof} Consider two vectors of CSPs $v_{1}$, $v_{2}$ such that $P(v_{1})$ and $P(v_{2})$ are both plausibly approachable. Assume for contradiction that we have some vector $v' = \alpha v_{1} + (1 - \alpha) v_{2}$ which is not plausibly approachable. This means that there exists some $q^{*} \in \Delta[m]$ and $d^{*} \in C_{\delta}$ such that 
\begin{align*}
    \max_{x \in P(v^{*}){\epsilon_{1}}}(d^{*})^{T}x < (d^{*})^{T}M(a,q^{*}) \ \ \forall a \in \Delta[n] 
\end{align*}


We can equivalently write the left hand side as
\begin{align*}
 \max_{x \in P(v^{*}){\epsilon_{1}}}(d^{*})^{T}x & = \max (d^{*})^{T}x \ \ s.t. \ \ x \cdot u_{j} \leq u_{j} \cdot v'[j], \ \ \forall j
 \\ &= \max (d^{*})^{T}x \ \ s.t. \ \ x \cdot u_{j} \leq u_{j} \cdot \alpha v_{1}[j] + u_{j} \cdot (1 - \alpha) v_{2}[j], \ \ \forall j \\
\end{align*}

Let $x^{*} =\argmax_{x} (d^{*})^{T}x \ \ s.t. \ \ x \cdot u_{j} \leq u_{j} \cdot \alpha v_{1}[j] + u_{j} \cdot (1 - \alpha) v_{2}[j], \ \ \forall j$. Then, we have that 

\begin{align*}
    (d^{*})^{T}x^{*} < (d^{*})^{T}M(a,q^{*}), \ \ \forall a \in \Delta[n] 
\end{align*}



However, we also have that 
\begin{align*}
     \max \alpha d_{i}^{T}x \ \ s.t. \ \ x \cdot u_{j} \leq u_{j} \cdot v_{1}[j] \ \ \forall j 
 \\ +  \max (1 - \alpha)d_{i}^{T}x \ \ s.t. \ \ x \cdot u_{j} \leq u_{j} \cdot v_{2}[j], \ \ \forall j \\
 \geq d_{i}^TM(a,q^{*}), \ \ \forall a \in \Delta[n]
\end{align*}

And 

\begin{align*}
    \max_{x \in P(v_{2}){\epsilon_{1}}}d_{i}^{T}x \geq d_{i}^{T}M(a,q^{*}) \ \ \forall a \in \Delta[n] \\
\end{align*}

\end{proof}


\begin{lemma} If $d + \delta_{1} \notin M$, then $d \notin M - \delta_{2}$
\end{lemma}

\begin{proof} If $d + \delta \notin M$, then $d \notin M$. If $d \notin M$, then $d \notin M - \delta$.
\end{proof}

\begin{theorem} There is a separation oracle 
\end{theorem}

\begin{theorem} LBMenu finds a valid menu $\M$ such that $V_{L}(\M,\phi) \geq V^{r}(\gamma)$ in time $f(m,n,k,\gamma)$.
\end{theorem}

\begin{proof}
LBMenu works as follows: it searches over points, constructs their menu, and asks

\end{proof}

\begin{theorem} UBValue computes $V^{UB}(\beta)$ such that $V^{opt}(\beta) \geq V^{UB}(\beta) \geq V^{max}$ in time $f(m,n,k,\beta)$.
\end{theorem}

\begin{proof}
\end{proof}


Structure of proof for optimal algorithm for a repeated game, given a prior over optimizer utilities of support size k.

\begin{itemize}
\item For every set of $k$ points in $mn$-dimensional space, there is a unique associated maximal polytope, defined by the incentive constraints matching each optimizer to a point. We only need to care about this polytope.
\item The idea is to search over the space of $k$ $mn$-dimensional points to optimize the expected utility of the learner. 
\item Is the search space the set of all k points in the $mn$-dimensional simplex? There are two feasibility conditions to satisfy, an individual rationality (IR) condition for mapping each realization of the optimizer's type to the corresponding point; and that the maximal polytope for this set is a valid menu, i.e., satisfies the individual rationality condition.
\item Given this definition of the search space, is it clear that it is convex?  One way to define a convex combination of two candidate elements (Each an ordered list of $k$ points) is to take their coordinate-wise convex combination - does this preserve the approachability property of the corresponding polytope? Have to check the algebra carefully. \textcolor{red}{Update}: Yes, it works out and the feasible set is indeed convex.

\item Does the Tsitsiklis et al. paper give us a membership oracle? Does the approximation there suffice? To check: If membership plus evaluation oracles suffice (the paper by Vempala et al. https://arxiv.org/abs/1706.07357). Note: Evaluating a set of k points is straightforward, but {\bf only} if it is within the feasible set -- do we also need a consistent notion of evaluation outside of the set? I think we can have a pseudo notion that is consistent.

\item Current concern: we are only given membership of a slightly altered convex set.
\end{itemize}


\esh{Status on Aug 29 : The email exchange shows us how to solve the general problem of optimal commitment; would be great if we could find a hardness proof}
 


==> backup/optimal_backup.tex <==
\section{Optimal General Commitment}
\label{sec:general}

%The main result of this section is establishing Theorem~\ref{thm:main_result_without_nr_alg} via proving an equivalent statement about menus.

\begin{theorem}
\label{thm:main_result_without_nr}
    There exists an algorithm (Algorithm~\ref{alg:d-opt-2}) running in time 
    
    $$O\left(\min \left\{ \poly \left(\frac{mn}{B\varepsilon}\right) \cdot 2^{\poly(k)}, \poly\left(
    \frac{k}{B\varepsilon}\right) \cdot 2^{\poly(mn)} \right\} \right)$$ 
    
    that constructs a $\varepsilon$-approximate optimal menu $\cM^\varepsilon$. We also show that this menu has a succinct description that is polynomially sized in $m$, $n$, and $k$.
\end{theorem}
%\esh{add B to the prelims?}


In searching for the optimal no-regret menu, Lemma~\ref{lem:decomp} showed that any no-regret menus can be replaced (in a way that preserved the payoffs of the learners and each possible optimizer) by a union of the no-swap-regret menu $\M_{NSR}$ and $k$-CSPs that correspond to the points in the menu selected by each optimizer type. This result was possible due to a characterization of no-regret menus showing all such menus contain $\M_{NSR}$ as a subset. Unfortunately, there is no such useful characterization for general menus. However, by focusing on the $k$ CSPs picked by each optimizer type, we show that all menus can be replaced by a polytope having a succinct description that preserves the payoff of the learner and each possible optimizer. Henceforth in this section, our solution space of objects is $\mathbb{R}^{mnk}$ and our points of interest are called k-CSPs and written in the standard form $\Phi = (\phi_1,\phi_2 \cdots \phi_k)$ where $\phi_i \in \mathbb{R}^{mn}$. We define the learner value of a k-CSP as $V_L(\Phi) := \sum_{i=1}^k \alpha_i u_L(\phi_i)$.


Of course not every k-CSP is realizable by an algorithm, since otherwise, we could make every CSP the one that maximizes the learner payoff. To address this issue, we associate each k-CSP with a polytope in $\mathbb{R}^{mn}$.

\begin{definition}[Canonical Polytope Operation]
\label{def:canonical}
The operation $\cC$ (defined below) converts a given k-CSP $\Phi$ into a polytope contained in the $mn$-dimensional simplex :

\[ \cC(\Phi) := \{ \phi \in \Delta^{mn} | u_{O,i}(\phi) \le u_{O,i}(\phi_i) \forall i \in [k] \}\]
    
\end{definition}

\begin{definition}[Canonical Polytope Operation, utility perspective]
\label{def:canonical_utility}
The operation $\cC_{}$ (defined below) converts a given k-CSP $\Phi$ into a polytope contained in the $k$-dimensional simplex :

\[ \cC_{v}(V) := \{ Q \in \Delta^{k} | Q_i \leq V_{i} \forall i \in [k] \}\]
    
\end{definition}

Armed with this definition, we can now restrict our interest to k-CSPs whose canonical polytope is a feasible menu.

\begin{definition}[Valid Menu k-CSPs]
The set $\cS$ (defined below) is the set of k-CSPs whose canonical polytope is a valid menu:

\[ \cS := \{ \Phi \in \Delta^{mnk} | \cC(\Phi) \text{ is a valid menu}.\}\]
    
\end{definition}



An immediate issue is that it is not even clear if the canonical polytope of a k-CSP $\Phi$ contains every CSP $\phi_i$ in the list.  In the failure of such an event, it is no longer possible for the $i$-th optimizer type to select CSP $\phi$ in $\cC(\Phi)$ (even if this set is a menu). Therefore, we add the following restriction to the set of k-CSPs.

\begin{definition}[Incentive Compatible Set]
The set $\cR$ (defined below) is the set of incentive compatible points:

\[ \cR := \{ \Phi \in \Delta^{mnk} | u_{O,i}(\phi_i) \ge u_{O,i}(\phi_j) \forall i,j \in [k] \}\]
    
\end{definition}

Our final feasible set is defined as their intersection.

\begin{definition}[Feasible Set]
The feasible set of k-CSPs $\cP$ is defined to be $\cP := \cR \cap \cS$.
    
\end{definition}


We present Algorithm~\ref{alg:d-opt-2} and spend the rest of the section to explaining it and proving the result of Theorem~\ref{thm:main_result_without_nr}.

\begin{algorithm}
\caption{Algorithm to Find the Optimal Commitment} \label{alg:d-opt-2}
\begin{algorithmic}[1]
    \STATE \textbf{Input:} A learner utility $u_{L}$ and a distribution over optimizer utilities $\mathcal{D}$.
    \STATE Use the membership oracle from Lemma~\ref{corollary:intersection_membership} and a convex optimization algorithm (see~\cite{lee2018efficient}) to find a point $X$ satisfying the following:
    \begin{itemize}
        \item $X \in \cR^\varepsilon \cap \cS^\varepsilon$
        \item $V_L(X) \ge \max_{Y \in \cR^\varepsilon \cap \cS^\varepsilon} V_L(Y) - \delta$
    \end{itemize}
    \STATE Identify a point $\Phi \in \cS$ with $\Phi = (\phi_1, \phi_2 \cdots \phi_k)$ such that $d(X,\Phi) \le \varepsilon$.
    \STATE{\bf Output} : $\cM := \text{Conv} \{\cC(\Phi) \cup \{\phi_1, \phi_2, \ldots, \phi_k\}\}$.
\end{algorithmic}
\end{algorithm}


As out first step, we show that there is an optimal menu that happens to be the canonical polytope of a k-CSP.

\begin{lemma}
    \label{lemma:succinct_opt_kcsp}
    There exists a k-CSP $\Phi^* \in \cR \cap \cS$ such that $V_L(\Phi^*) = V_L(\cC(\phi^*))$ where $\cC(\phi^*)$ is an optimal menu to commit to when playing against a prior $\cD$ of optimizers.
\end{lemma}

\begin{proof}
    Consider an optimal menu $\cM^*$. Let $\phi_1$, $\phi_2 , \cdots \phi_k$ be the CSPs ``chosen" by optimizer type $i$ in the menu $\cM^*$. Our candidate k-CSP $\Phi$ is the ordered tuple of these $k$-CSPs $\phi_1$ to $\phi_k$. Tautologically, $u_{O,i}(\phi_i) \ge u_{O,i}(\phi_j)$ for each $i,j \in [k]$, implying that $\Phi \in \cR$. To show that $\Phi \in \cS$, we show that $\cM^* \subseteq \cC(\Phi)$, since menus are upwards closed, this would complete the proof. Consider any CSP $\phi \in \cM^* \subseteq \Delta^{mn}$ and any $i \in [k]$, since the i-th optimizer weakly prefers $\phi_i$, we have $u_{O,i} (\phi_i) \ge u_{O,i}(\phi)$. Thus, this $\phi$ satisfies all the constraints required to be satisfied to be present in the polytope $\cC(\Phi)$, which finishes this proof. 
\end{proof}

Next, we show that the sets $\cR$ and $\cS$ are convex and that their intersection is non-empty.


\begin{observation}
    The set $\cP$ is non-empty.
\end{observation}

\begin{proof}
    $\Phi^* = (\phi_1^*,\phi_2^*,\cdots \phi_k^*) \in \cP$ where $\phi^*_i \in \argmax_{\phi in \Delta^{mn}} u_{O,i}(\phi)$. This is because we tautologically satisfy the conditions in $\cR$ while containment in $\cS$ follows from the fact that $\cC(\Phi^*) = \Delta^{mn}$.
\end{proof}

\begin{comment}
    

\begin{observation}
    The set $\cP^\varepsilon$ contains a $\varepsilon$-ball in $mn$-dimensional space.
\end{observation}
\end{comment}

\begin{lemma}
\label{lem:S_is_convex}
    The set $\cS$ is convex.
\end{lemma}



\begin{lemma}
\label{lem:R_is_convex}
    The set $\cR$ is convex.
\end{lemma}


We need one final technical lemma, about a membership oracle for the set $\cR \cap \cS$, to prove the main 
result of this section. 

\begin{lemma}
\label{corollary:intersection_membership}
    There is an algorithm with running time $\min \left\{ \text{Poly}(\frac{mn}{\varepsilon}) \cdot 2^{\text{Poly}(k)}, \text{Poly}(\frac{k}{\varepsilon}) \cdot 2^{\text{Poly} (mn)}\right\}$ that is a $\varepsilon$-membership oracle for the (convex) set $\cR^\varepsilon \cap \cS^\varepsilon$.
\end{lemma}

The proof of this lemma is provided at the end of the section.


%Finally, we also demonstrate that there 

\subsection{Proof of Theorem~\ref{thm:main_result_without_nr}}
%\esh{editing}

Since the sets $\cR$ and $\cS$ are convex, the intersection of their expansions is also convex. Lemma~\ref{corollary:intersection_membership} gives us a membership oracle for the $\cR^\varepsilon \cap \cS^\varepsilon$ and we have already defined a valuation oracle for each $k$-CSP. Thus, employing an algorithm to optimize a linear function in a convex set (see~\cite{lee2018efficient}) gives us $x \in \cR^\varepsilon \cap \cS^\varepsilon$ such that $V_L(x) \ge \max_{y \in \cR^\varepsilon \cap \cS^\varepsilon} V_L(y) - \delta$.

Since $x \in \cR^\varepsilon \cap \cS^\varepsilon$, there exist points $ r \in \cR$ and $s \in \cS$ such that $d(x,r) \le \varepsilon$ and $d(x,s) \le \varepsilon$. We claim that this point $x$ can be efficiently found by perturbing each CSP in $x$ in the direction of higher payoff for the corresponding optimizer type -- this procedure is outlined in Algorithm~\ref{alg:water}.

The triangle inequality gives $d(r,s) \le 2 \varepsilon$. Since all the payoff vectors are within the bounds $[-1,1]^{mn}$, $V_L(s) \ge V_L(x) -2\sqrt{mn}\varepsilon \ge V^* - (2\sqrt{mn}\varepsilon+\delta)$.


Write $s  = (\phi_1, \phi_2 \cdots \phi_k)$ and $r  = (\phi'_1, \phi'_2 \cdots \phi'_k)$. Since $d(r,s) \le 2 \varepsilon$, $u_{O,i}(\phi_i) \ge u_{O,i}(\phi'_i) -  2 \sqrt{mn}\varepsilon $ and $u_{O,i}(\phi_j) \le u_{O,i}(\phi'_j) +  2\sqrt{mn} \varepsilon $ for all $i,j \in [k]$. However, since $r \in \cR$, $u_{O,i}(\phi'_i) \ge u_{O,i}(\phi'_j)$, thus we get $u_{O,i}(\phi_i) \ge u_{O,i}(\phi_j) - 4 \sqrt{mn}\varepsilon$ for all $i,j \in [k]$ ,i.e., the incentive compatibility constraints are approximately satisfied by the point $s$. Construct the set $\cM : = \text{Conv} \{\cC(s) \cup \{\phi_1,\phi_2 \cdots \phi_k\} \}$. First, we see that $\cM$ is a feasible menu, since $\cC(s)$ is a feasible menu (due to $s \in \cS$) and menus are upwards closed~\ref{corollary:upwards_closed}. Second, we see that $u_{O,i}(\phi_i) \ge u_{O,i}(\phi) - 4 \sqrt{mn} \varepsilon$ for all $\phi \in \cM$ (using the properties of $\cC$ and the inequalities proved in the last step). If the optimizer type is willing to take a hit of up to $4 \sqrt{mn}\varepsilon$ while best-responding in the menu $\cM$, the point $p_i$ picked by the $i$-th optimizer satisfies $u_L(p_i) \ge u_L(\phi_i)$ since we have just shown that $\phi_i$ is a candidate point for the $i$-th optimizer type.

Thus, $V^{4 \sqrt{mn} \varepsilon}_L(\cM) \ge V_L(S) \ge V^* - (2 \sqrt{mn} \varepsilon + \delta)$. The optimization algorithm of~\cite{lee2018efficient} 
makes polynomial in $\frac{mnk}{\varepsilon}$ number of calls to the membership oracle for the set $\cR$ and $\cS$. Applying the running time bound of this membership oracle with a suitable value of $\varepsilon$ completes the proof.

\subsection{Proof of Lemma~\ref{corollary:intersection_membership}}

The definition of $\cR$ admits a straighforward membership oracle, based upon checking the CSP constraints and $n \choose 2$ inequalities.
\begin{lemma}
    \label{lemma:ic_membership}
    There is a polynomial time membership oracle for the set $\cR$.
\end{lemma}

On the other hand, verifying membership in $\cS$ is an altogether trickier problem, since it entails algorithmically certifying that the canonical polytope of the given k-CSP is a menu. We introduce some technical tools developed by~\cite{mannor2009approachability} for verifying the approachability of a convex set of payoff vectors for a given vector valued game and demonstrate that these can be used to address membership queries in $\cS$. 

\begin{theorem}[~\cite{mannor2009approachability}]
\label{thm:tsitsiklis}
    There is an algorithm with running time $\min \left\{ \text{Poly}(\frac{mn}{\varepsilon}) \cdot 2^{\text{Poly}(k)}, \text{Poly}(\frac{k}{\varepsilon}) \cdot 2^{\text{Poly} (mn)}\right\}$ which, given a polytope $D$ in $mn$ dimensional space with a $poly(mnk)$ (running time) membership oracle and a given $k$-dimensional vector valued game between two players with $m$ and $n$ actions each, correctly outputs one of the following two results:
    \begin{itemize}
        \item $D^{\epsilon}$ is approachable
        \item $D$ is not approachable
    \end{itemize}
\end{theorem}

We use this result to construct two different membership oracle for $\cS^\varepsilon$, one of which runs in polynomial time in $m,n, \frac{1}{\varepsilon}$ for constant $k$ and the other in polynomial time in $k, \frac{1}{\varepsilon}$.

\begin{theorem}
\label{thm:approachability_oracle}
    There is an algorithm with running time $ \text{Poly}(\frac{k}{B\varepsilon}) \cdot 2^{\text{Poly} (mn)}$ that is a $\varepsilon$-membership oracle for the set $\cS$. 
\end{theorem}

\begin{proof}
The algorithm operates as follows: given some k-CSP $\Phi$, compute the result of \ref{thm:tsitsiklis} for the set $C(\Phi)$ on the Menu approachability game defined in Defintion~\ref{def:menu_game_a} using the approximation parameter of $\epsilon' = \frac{B\epsilon}{k\sqrt{mn}}$. This will reveal either that $C(\Phi)^{\epsilon'}$ is approachable, or $C(\Phi)$ is not approachable. In the first case, our algorithm outputs that $\Phi \in \cS^{\epsilon}$. in the second case, our algorithm outputs that $\Phi \notin \cS$.


First, we will show that if $C(\Phi)^{\epsilon'}$ is approachable, then $\Phi \in \cS^{\epsilon}$. For the purposes of this section of the proof, we will assume that $C(\Phi)^{\epsilon'}$ is approachable. Now, consider a new polytope $M$, defined as follows: 
\[ M := \left\{ \phi \in \Delta^{mn} | u_{O,i}(\phi) \le u_{O,i}(\Phi_i) + \frac{B\epsilon}{k}, \forall i \in [k] \right\}\]

We will prove that $C(\Phi)^{\epsilon'} \subseteq M$.  To see this, consider any CSP $\phi^{*}$ in $C(\Phi)^{\epsilon'}$. Then, we have that 
$$\inf_{\phi \in C(\Phi)}||\phi^{*} - \phi||_{2} \leq \epsilon'$$

Because $C(\Phi)$ is a polytope and therefore closed, we can consider some $\phi^{**} \in C(\Phi)$ such that $||\phi^{*} - \phi^{**}||_{2} \leq \epsilon'$. We therefore have that  

$$ u_{O,i}(\phi^{**}) \le u_{O,i}(\Phi_i), \forall i \in [k]$$

And therefore that, for all $i$, 
\begin{align*}
  & ||\phi^{*} - \phi^{**}||_{2} \leq \epsilon' = \frac{B\epsilon}{k\sqrt{mn}}  \\
  & \implies u_{O,i}(\phi^{*}) - u_{O,i}(\phi^{**}) \leq \frac{B \epsilon}{k} \tag{By Cauchy-Schwartz and the fact that $u_{O,i} \in [-1,1]$}  \\
& \implies u_{O,i}(\phi^{*}) \leq u_{O,i}(\Phi_i) +  \frac{B\epsilon}{k}  \tag{By the fact that $u_{O,i}(\phi^{**}) \le u_{O,i}(\Phi_i), \forall i \in [k]$}  
\\ & \implies \phi^{*} \in M
\end{align*}

We have shown that $C(\Phi)^{\epsilon'} \subseteq M$. Therefore, by the upwards-closedness of menus shown in Corollary~\ref{corollary:upwards_closed}, since $C(\Phi)^{\epsilon'}$ is approachable, then $M$ is approachable. Now, let us consider $M'$, a subset of $M$, defined as follows:
\[ M' := \left\{ \phi \in \Delta^{mn} | u_{O,i}(\phi) \le \min(u_{O,i}(\Phi_i) + \frac{B\epsilon}{k}, L+_{i}), \forall i \in [k] \right\}\]

As $M$ is approachable, let $\cA$ be the algorithm which runs Blackwell approachability on the set $M$. Note that regardless of what the optimizer plays, it is not possible to obtain points $\phi$ such that $u_{O,i}(\phi) > L+_{i}$. Therefore, the menu of $\cA$ must be strictly contained within $M'$. Thus, $M'$ is also approachable.

Now, consider the k-CSP $\Phi^{*}$ which strictly increases the utility of every agent by $\frac{B \epsilon}{k}$ in the following way: let $i(1),...,i(mn)$ index the move pairs in increasing order of learner utility $i$. Then, we construct $\Phi^{*}$ as in Algorithm~\ref{alg:water}.

\begin{algorithm}
\caption{Water-Filling Algorithm for Constructing $\Phi^*$} \label{alg:water}
\begin{algorithmic}[1]
    \STATE \textbf{Input:} A point $\Phi \in \cS^\varepsilon$
    \STATE \textbf{Output:} A $k$-CSP $\Phi^* \in \cS$
    
    \FOR{$i = 1$ to $k$}
        \STATE Initialize $w \gets 0$
        \STATE Initialize $j \gets 1$
        \WHILE{$w < \frac{\epsilon}{k}$ \AND $j \leq mn$}
            \STATE Update $\Phi^{*}_{i}[i(j)] \gets \max\left(0, \Phi_{i}[i(j)] - \frac{\epsilon}{k} + w\right)$
            \STATE Update $w \gets w + \Phi_{i}[i(j)] - \Phi^{*}_{i}[i(j)]$
            \STATE Increment $j \gets j + 1$
        \ENDWHILE
        \STATE Set the last entry $\Phi^{*}_{i}[i(mn)] \gets \Phi_{i}[i(mn)] + w$
    \ENDFOR
\end{algorithmic}
\end{algorithm}


Informally: for every $i$, for $\Phi_{i}$, we decrease the weight on the worst move pairs for agent $i$ (not going below zero) until the total weight has been decreased by $\frac{\epsilon}{k}$ or we run out of move pairs, and then we increase the weight on $L+_{i}$ by the total amount decreased. In doing this, for every $i$, there are two possibilities:
\begin{itemize}
    \item There is at least $\frac{\epsilon}{k}$ weight on action pairs in $\Phi$ that are not $L+_{i}$. Then, $u_{O,i}(\Phi_{i}^{*}) > u_{O,i}(\Phi_{i}) + \frac{B\epsilon}{k}$, where $B$ is the smallest gap between utilities in the game. 
    \item $\Phi_{i}^{*} = L+$. 
\end{itemize}

Thus, we have that for all $i$, $u_{O,i}(\Phi^{*}_{i}) \geq \min(u_{O,i}(\Phi_i) + \frac{B\epsilon}{k}, L+_{i})$. Therefore, $C(\Phi^{*}) \supseteq M'$, and since $M'$ is approachable, $C(\Phi^{*})$ is approachable. Therefore, $\Phi^{*} \in \cS$. 

Now, note that the $\ell_1$-distance between $\Phi^{*}$ and $\Phi$ is at most $k \cdot \frac{\epsilon}{k} = \epsilon$, by construction, and this upper bounds the $\ell_2$ distance. Furthermore, recall that $\Phi^{*} \in \cS$. Therefore, $\Phi \in \cS^{\epsilon}$. 



Finally, we must show that, if $C(\Phi)$ is not approachable, then $\Phi \notin \cS$. But this follows directly from the definition of $\cS$, so we are done.

Using the algorithm in Theorem~\ref{thm:tsitsiklis} with $\epsilon' = \frac{B\epsilon}{k\sqrt{mn}}$, the total runtime is 
\begin{align*}
  &   \poly\left(\frac{k}{\epsilon'}\right)\cdot 2^{\poly(mn)} \\
  & = \poly \left(\frac{k^{2}\sqrt{mn}}{B \epsilon}\right)\cdot 2^{\poly(mn)} \\
  & = \poly\left(\frac{k}{B \epsilon}\right) \cdot 2^{\poly(mn)}
\end{align*}



\end{proof}

%\esh{@Natalie, let's work on the final result here}
A similar sequence of ideas is used to obtain an algorithm with a polynomial dependence on $mn$, at the cost of an exponential dependence on $k$. The main difference lies in working with a $k$-dimensional vector valued game that corresponds to the payoffs obtained by each optimizer type. The proof of the theorem below can be found in the Appendix.
\begin{theorem}
\label{thm:approachability_oracle2}
    There is an algorithm with running time $ \poly\left(\frac{mn}{B\varepsilon}\right) \cdot 2^{\poly(k)}$ that is a $\varepsilon$-membership oracle for the set $\cS$. 
\end{theorem}


\subsection{Hardness of Menu Testing}

While our algorithm finds an optimal commitment efficiently for small games and constant number of optimizer types, our procedure dos not run in time polynomial in the number of actions and the number of types simultaneously. We show that our algorithmic approach would require significant alterations to produce such a result via demonstrating a hardness barrier.

A key element of our result for finding optimal algorithmic commitments was using the algorithm of~\cite{mannor2009approachability} to check if a given polytope is Blackwell approachable (for an arbitrary vector valued game).~\cite{mannor2009approachability} showed that this problem is NP-hard in general. We extend this result by showing that testing the approachability of a given convex set remains NP-hard even when the set is a canonical polytope (see definition~\ref{def:canonical}), which is exactly the class of our problem our algorithmic approach requires us to solve.



\begin{comment}
    

\begin{theorem}[Informal]

Testing if the polytope induced by a $k$-CSP is  NP-hard.
    
\end{theorem}
\end{comment}
\begin{theorem}
\label{thm:hardness}
The problem of checking if the canonical polytope $\cC(\Phi)$ of a given $k$-CSP $\Phi$ for an arbitrary vector valued game is NP-hard.
\end{theorem}

The proof (in Appendix~\ref{app:hardness}) follows straightforwardly from a proof in~\cite{mannor2009approachability} about the hardness of testing approachability of the non-negative orthant.



==> backup/optimal_old.tex <==
\section{Without the No-Regret Condition - Old }

\begin{comment}
    

We consider a setting where two players, an \emph{optimizer} $O$ and a \emph{learner} $L$, repeatedly play a two-player bimatrix game $G$ for $T$ rounds. The game $G$ has $m$ actions for the optimizer and $n$ actions for the learner, and is specified by two bounded payoff functions $u_{O}: [m] \times [n] \rightarrow [-1, 1]$ (denoting the payoff for the optimizer) and $u_{L}: [m] \times [n] \rightarrow [-1, 1]$ (denoting the payoff for the learner). During each round $t$, the optimizer picks a mixed strategy $x_t \in \Delta_{m}$ while the learner simultaneously picks a mixed strategy $y_{t} \in \Delta_{n}$; the learner then receives reward $u_{L}(x_t, y_t)$ and the optimizer receives reward $u_{O}(x_t, y_t)$ (where here we have linearly extended $u_{L}$ and $u_{O}$ to take domain $\Delta_{m} \times \Delta_{n}$). Both the learner and optimizer observe the full mixed strategy of the other player (the ``full-information'' setting).

The learner will employ a \emph{learning algorithm} $\cA$ to decide how to play. For our purposes, a learning algorithm is a family of horizon-dependent algorithms $\{A^T\}_{T \in \mathbb{N}}$. Each $A^{T}$ describes the algorithm the learner follows for a fixed time horizon $T$. Each horizon-dependent algorithm is a mapping from the history of play to the next round's action, denoted by a  collection of $T$ functions $A^T_1, A^T_2 \cdots A^T_T$, each of which deterministically map the transcript of play (up to the corresponding round) to a mixed strategy to be used in the next round, i.e., $A^T_t(x_1, x_2,\cdots, x_{t-1}) = y_t$. 

We assume that the learner is able to see $u_{L}$ before committing to their algorithm $\cA$, but has only a prior $\phi$ over $u_O$. We further assume that $\phi$ has finite support $k$. Formally, 

\begin{definition}[Prior $\cD$] $\cD$ is a $k$-dimensional vector of tuples such that $\cD[i] = (u_{i}, p_{i})$, signifying that the optimizer has probability $p_{i}$ of having utility $u_{i}$. We also let $\cD^{u}$ refer to only the vector of utilities, and similarly we let $\cD^{p}$ refer only to the vector of probabilities. Finally, we will abuse notation and sometimes refer to the support of the distribution as $\cD$.
\end{definition}

 The optimizer, who knows $u_L$ and $u_{O}$, will approximately best-respond by selecting a sequence of actions that approximately (up to sublinear $o(T)$ factors) maximizes their payoff. They break ties in the learner's favor. Formally, for each $T$ let

\begin{equation*}
    V_{O}(\cA, u_O, T) = \sup_{(x_1, \dots, x_T) \in \Delta_{m}^{T}} \frac{1}{T}\sum_{t=1}^{T} u_{O}(x_t, y_t)
\end{equation*}

\noindent
represent the maximum per-round utility of the optimizer with payoff $u_O$ playing against $\cA$ in a $T$ round game (here and throughout, each $y_t$ is determined by running $A^{T}_{t}$ on the prefix $x_1$ through $x_{t-1}$). For any $\eps > 0$, let 

\begin{equation*}
\cX(\cA, u_O, T, \eps) = \left\{(x_1, x_2, \dots, x_T) \in \Delta_{m}^T \bigm| \frac{1}{T}\sum_{t=1}^{T} u_{O}(x_t, y_t) \geq V_{O}(\cA, u_O, T) - \eps \right\}
\end{equation*}

\noindent
be the set of $\eps$-approximate best-responses for the optimizer to the algorithm $\cA$. Finally, let

\begin{equation*}
V_{L}(\cA, u_O, T, \eps) = \sup_{(x_1, \dots, x_T) \in \cX(\cA, u_O, T, \eps)} \frac{1}{T}\sum_{t=1}^{T} u_{L}(x_t, y_t)
\end{equation*}

\noindent
represent the maximum per-round utility of the learner under any of these approximate best-responses if the follower's utility is $u_{O}$. 

We are concerned with the asymptotic per-round payoff of the learner as $T \rightarrow \infty$ and $\eps \rightarrow 0$. Specifically, let

\begin{equation}\label{eq:learner_value}
V_{L}(\cA, u_O) = \lim_{\eps \rightarrow 0} \liminf_{T \rightarrow \infty} V_{L}(\cA, u_O, T, \eps).
\end{equation}

\noindent
Note that the outer limit in \eqref{eq:learner_value} is well-defined since for each $T$, $V_{L}(A, u_O, T, \eps)$ is decreasing in $\eps$ (being a supremum over a smaller set). 

The learner would like to select a learning algorithm that maximizes their own asymptotic per-round payoff in expectation over their prior $\cD$, which we define as

\begin{equation*}
V_{L}(\cA, \cD) = \sum_{u_{O} \sim \cD}V_{L}(\cA, u_{O}) \cdot Pr(\cD = u_{O})
\end{equation*}

\end{comment}



    

\esh{Note to self: add in preliminaries for menus}

Our problem can equivalently stated in the following terms -- the learner picks a menu $\cM$ in $mn$-dimensional space and gets value:

\begin{equation*}
V_{L}(\cM, \cD) = \sum_{u_{O} \sim \cD}V_{L}(\cM, u_{O}) \cdot Pr(\cD = u_{O})
\end{equation*}
Therfore the objective of the learner is to pick a menu from the set $\cM^*$ defined as

\[
\cM^* = \argmax_{\cM \in \cF} \sum_{u_{O} \sim \cD}V_{L}(\cM, u_{O}) \cdot Pr(\cD = u_{O})
\]

where $\cF$ is the set of realizable or feasible menus in $mn$-dimensional space. Let $V^* = V_L(\cM^*, \cD)$.


\esh{Define an $\epsilon$-menu $\mathcal{M}_\varepsilon$ in the preliminaries, corresponding to the optimizer best-responding suboptimally upto $\varepsilon$ to favor the learner}

We solve a slightly easier version of the original problem, where we expand our search over menus to include $\epsilon$-menus. Our main result is as follows --

\begin{theorem}
\label{thm:main_result_without_nr}
    There exists a procedure running in time $\min \{ \text{Poly}(mn) \cdot 2^{\text{Poly}\left (k/\varepsilon \right)}, \text{Poly}(k) \cdot 2^{\text{Poly}\left (mn/\varepsilon \right)}\}$ that constructs a $\varepsilon$-menu $\cM^\varepsilon$ such that $V^\varepsilon_L(\cM^\varepsilon, \cD) \ge V^* - \varepsilon$.
\end{theorem}

We also show that this menu has a succinct description that is polynomially sized in $m,n,k$.



\subsection{Geometric Preliminaries}

\esh{move these two definitions to prelims?}
\begin{definition}[Point-to-set Distance] For some point $x$ in $\mathbb{R}^{d}$ and some convex set $D$ in $\mathbb{R}^{d}$, let the point-to-set distance $\rho(x,D) = \inf_{y \in D}||x - y||_2$.
\end{definition}

\begin{definition}[$\epsilon$-Expansion and $\epsilon$-contraction of a Set] Consider some set $D \in \mathbb{R}^{d}$. The $\epsilon$-expansion of $D$ is the set $D^{\epsilon}$ such that
\begin{equation}
    D^{\epsilon} = \{x : \rho(x,D) \leq \epsilon \}
\end{equation}

Conversely, $D$ is the $\epsilon$-contraction of $D^{\epsilon}$.
\end{definition}

\esh{Natalie has a good point about this exercise also working if the drawn type affects the learner's payoff in both cases of whether they get to observe it or not}

\begin{definition}[The Optimizer]
    The optimizer is characterized by a public prior distribution $D$ on functions that map $\Delta^{mn} \rightarrow [-1,1]$. $D$ has support $k$, and puts probability $\alpha_i$ on payoff function $u_{O,i}$ for $i \in [k]$.
\end{definition}


The search space is over $\mathbb{R}^{mnk}$, we write points of interest, called k-CSPs in the standard form $\Phi = (\phi_1,\phi_2 \cdots \phi_k)$ where $\phi_i \in \mathbb{R}^{mn}$.


\esh{Maybe we should not use $V_L$ here, even though it is almost the same thing as the usual $V_L$, the equivalence breaks when we go outside $\cP$.}
\begin{definition}[Learner Value Function]
The learner value of a candidate solution $\phi$ is $V_L(\Phi) := \sum_{i=1}^k \alpha_i u_L(\phi_i)$.
\end{definition}

\begin{definition}[Incentive Compatible Set]
The set $\cR$ (defined below) is the set of incentive compatible points:

\[ \cR := \{ \Phi \in \Delta^{mnk} | u_{O,i}(\phi_i) \ge u_{O,i}(\phi_j) \forall i,j \in [k] \}\]
    
\end{definition}

We define a canonical operation that takes any k-CSP $\Phi$ and converts it into the following polytope.

\begin{definition}[Canonical Polytope Operation]
The operation $\cC$ (defined below) converts a given k CSP set $\phi$ into a polytope contained in the $mn$-dimensional simplex :

\esh{Might want to union the original points as well with a convex hull, especially in the case with approximation}

\[ \cC(\Phi) := \{ \phi \in \Delta^{mn} | u_{O,i}(\phi) \le u_{O,i}(\phi_i) \forall i \in [k] \}\]
    
\end{definition}

\esh{Once we define menus, we should make this definition formal.}
\begin{definition}[Valid Menu k-CSPs]
The set $\cS$ (defined below) is the set of k-CSPs whose canonical polytope is a valid menu:

\[ \cS := \{ \Phi \in \Delta^{mnk} | \cC(\Phi) \text{ is a valid menu}.\}\]
    
\end{definition}

\begin{definition}[Feasible Set]
The feasible set of k-CSPs $\cP$ is defined to be $\cP := \cR \cap \cS$.
    
\end{definition}

Rethinking the search space in terms of k-CSPs is justified by the following lemma, which shows that an optimal commitment menu can be written as the canonical polytope operation applied on a particular k-CSP.


\begin{lemma}
    \label{lemma:succinct_opt_kcsp}
    There exists a k-CSP $\Phi^*$ such that $V_L(\Phi^*) = V_L(\cM^*)$ where $\cM^*$ is an optimal menu to commit to when playing against a prior $\cD$ of optimizers.
\end{lemma}

\begin{proof}
    Consider an optimal menu $\cM^*$. Let $\phi_1$, $\phi_2 , \cdots \phi_k$ be the CSPs ``chosen" by optimizer type $i$ in the menu $\cM^*$. Our candidate k-CSP $\Phi$ is the ordered tuple of these $k$-CSPs $\phi_1$ to $\phi_k$. Tautologically, $u_{O,i}(\phi_i) \ge u_{O,i}(\phi_j)$ for each $i,j \in [k]$, implying that $\Phi \in \cR$. To show that $\Phi \in \cS$, we show that $\cM^* \subseteq \cC(\Phi)$, since menus are upwards closed, this would complete the proof. Consider any CSP $\phi \in \cM^* \subseteq \Delta^{mn}$ and any $i \in [k]$, since the i-th optimizer weakly prefers $\phi_i$, we have $u_{O,i} (\phi_i) \ge u_{O,i}(\phi)$. Thus, this $\phi$ satisfies all the constraints required to be satisfied to be present in the polytope $\cC(\Phi)$, which finishes this proof. 
\end{proof}

Thus the original problem of this section can be rewritten as finding $\Phi \in \argmax_{\Phi \in \cP} V_L(\Phi)$.

\esh{Ending the new defs here}




\section{Preliminaries}

\begin{observation}
    The set $\cP$ is non-empty.
\end{observation}

\begin{proof}
    $\Phi^* = (\phi_1^*,\phi_2^*,\cdots \phi_k^*) \in \cP$ where $\phi^*_i \in \argmax_{\phi in \Delta^{mn}} u_{O,i}(\phi)$. This is because we tautologically satisfy the conditions in $\cR$ while containment in $\cS$ follows from the fact that $\cC(\Phi^*) = \Delta^{mn}$.
\end{proof}

\begin{observation}
    The set $\cP^\varepsilon$ contains a $\varepsilon$-ball in $mn$-dimensional space.
\end{observation}


\begin{lemma}
    The set $\cS$ is convex.
\end{lemma}
\begin{proof}
Consider two k-CSPs $\Phi^{1}$ and $\Phi^{2}$ such that $C(\Phi^{1})$ and $C(\Phi^{2})$ are both valid menus. Let $\Phi' = \alpha \Phi^{1} + (1-\alpha)\Phi^{2}$. Then, our goal is to prove that $C(\Phi')$ is a valid menu. To do this, we will propose a candidate algorithm which has a menu contained within $C(\Phi')$. Let us refer to $\A_{1}$ as an algorithm with the menu $C(\Phi^{1})$ and $\A_{2}$ as an algorithm with the menu $C(\Phi^{2})$. These algorithms must exist, given our assumptions that $\Phi^{1}$ and $\Phi^{2}$ are in $\cS$. Then our new algorithm $\A'$ is as follows. It will initialize algorithms $\A_{1}$ and $\A_{2}$. Then, at each time step $t$ given a sequence of optimizer actions so far $s^{1:t}$, it will play $\alpha \A_{1}(s^{1:t}) + (1 -\alpha) \A_{2}(s^{1:t})$. We claim that $\M(\A') \subseteq C(\Phi')$, and therefore that $C(\Phi')$ is a menu. 
Let us assume for contradiction that this is not the case. Then, there is a sequence $s$ that the optimizer can play such that the resulting CSP is not in $C(\Phi')$. Note that $C(\Phi')$ is the set of all CSPs $x$ such that, for all $i$, $u_{O,i}(\Phi'_i) \geq u_{O,i}(x)$. Thus, there is a sequence that the optimizer can play against $\A'$ such that in the resulting CSP $x$, there is some $i$ s.t. $u_{O,i}(\Phi'_i) < u_{O,i}(x)$. So we have

\begin{align*}
u_{O,i}(\Phi'_i) < u_{O,i}(\A'(s)) &
\\ & \implies u_{O,i}(\alpha \Phi^{1}_{i} + (1 - \alpha) \Phi^{2}_{i}) < u_{O,i}(\A'(s)) \\
& \implies u_{O,i}(\alpha \Phi^{1}_{i} + (1 - \alpha) \Phi^{2}_i) < u_{O,i}(\alpha \A_{1}(s) + (1 - \alpha)\A_{2}(s)) \tag{By the definition of $\A'$} \\
& \implies \alpha u_{O,i}(\Phi^{1}_i) + (1 - \alpha) u_{O,i}(\Phi^{2}_i) < \alpha u_{O,i}(\A_{1}(s)) + (1 - \alpha)u_{O,i}(\A_{2}(s)) \tag{By the linearity of $u_{O,i}$} \\
& \implies \alpha (u_{O,i}(\Phi^{1}_i) - u_{O,i}(\A_{1}(s)))  <  (1 - \alpha)(u_{O,i}(\A_{2}(s)) - u_{O,i}(\Phi^{2}_i))  \\
& \implies \alpha (0)  <  (1 - \alpha)(u_{O,i}(\A_{2}(s)) - u_{O,i}(\Phi^{2}_i)) \tag{By the definition of $\A_{1}$} \\
& \implies \alpha (0)  <  (1 - \alpha)(0) \tag{By the definition of $\A_{2}$} \\
\end{align*}

This derives a contradiction. Therefore the menu of $\A'$ is contained within $C(\Phi')$. By the upward-closedness of menus given in Corollary~\ref{corollary:upwards_closed}, $C(\Phi')$ is also a valid menu, and therefore $\Phi' \in S$.
\end{proof}


\begin{lemma}
    The set $\cR$ is convex.
\end{lemma}
\begin{proof}
    Consider two k-CSPs $\Phi^{1}$ and $\Phi^{2}$ such that $\Phi^{1}$ and $\Phi^{2}$ are in $\cR$. Then, our goal is to prove that $\Phi' = \alpha \Phi^{1} + (1-\alpha)\Phi^{2}$ is in $\cR$. Assume for contradiction that this is not the case. Then, there is some $(i,j)$ pair such that 
    
\begin{align*}
 u_{O,i}(\Phi'_{i}) < u_{O,i}(\Phi'_{j}) \\
& \implies u_{O,i}(\alpha \Phi^{1}_i + (1 - \alpha) \Phi^{2}_i) < u_{O,i}(\alpha \Phi^{1}_j + (1 - \alpha) \Phi^{2}_j) \\
& \implies \alpha u_{O,i}(\Phi^{1}_i) + (1 - \alpha) u_{O,i}(\Phi^{2}_i) < \alpha u_{O,i}(\Phi^{1}_j) + (1 - \alpha) u_{O,i}(\Phi^{2}_j) \tag{By the linearity of $u_{O,i}$} \\
& \implies \alpha (u_{O,i}(\Phi^{1}_i) -  u_{O,i}(\Phi^{1}_j)) < (1 - \alpha) (u_{O,i}(\Phi^{2}_j)  - u_{O,i}(\Phi^{2}_i)) \\
& \implies \alpha (0) < (1 - \alpha) (0) \tag{By the fact that $\Phi^{1}$ and $\Phi^{2}$ are in $\cR$} \\
\end{align*}

This derives a contradiction, and therefore $\Phi'$ is also in $\cR$.

\end{proof}


\esh{Might not need this lemma below - besides it's not even true!} \nat{lol can we delete it then}
\begin{lemma}[\esh{Folklore? - we need a reference}]
If $A = B \cap C$ where $B,C$ are convex sets for $A,B,C \subseteq \mathbb{R}^n$ for some integer $n$, then 
$B^{\frac{\varepsilon}{2}} \cap C^{\frac{\varepsilon}{2}} \subseteq A^\varepsilon$.    
\end{lemma}

\begin{lemma}
\label{lemma:wlog_polytope}
    Recall that $V^*$ is the expected value of the optimal learner commitment algorithms -- there exists $\Phi \in \cP$ such that $V_L(\Phi) = V^*$. Further, the same $\Phi$ has the property that $\cC(\Phi)$ is the optimal menu for the learner to commit to.
\end{lemma}

\section{Results}

\esh{New chain of results to prove Theorem~\ref{thm:main_result_without_nr}}

\begin{theorem}[~\cite{mannor2009approachability}]
\label{thm:tsitsiklis}
    There is an algorithm with running time $\min \left\{ \text{Poly}(\frac{mn}{\varepsilon}) \cdot 2^{\text{Poly}(k)}, \text{Poly}(\frac{k}{\varepsilon}) \cdot 2^{\text{Poly} (mn)}\right\}$ which, given a polytope $D$ in $mn$ dimensional space with $poly(k)$ membership oracle, correctly outputs one of the following two results:
    \begin{itemize}
        \item $D^{\epsilon}$ is approachable
        \item $D$ is not approachable
    \end{itemize}
\end{theorem}

\begin{theorem}
\label{thm:approachability_oracle}
    There is an algorithm with running time $ \text{Poly}(\frac{k}{B\varepsilon}) \cdot 2^{\text{Poly} (mn)}$ that is a $\varepsilon$-membership oracle for the set $\cS$. 
\end{theorem}

\begin{proof}
The algorithm operates as follows: given some k-CSP $\Phi$, compute the result of \ref{thm:tsitsiklis} for the set $C(\Phi)$ on the Menu approachability game defined in Defintion~\ref{def:menu_game_a} using the approximation parameter of $\epsilon' = \frac{B\epsilon}{k\sqrt{mn}}$. This will reveal either that $C(\Phi)^{\epsilon'}$ is approachable, or $C(\Phi)$ is not approachable. In the first case, our algorithm outputs that $\Phi \in \cS^{\epsilon}$. in the second case, our algorithm outputs that $\Phi \notin \cS$.


First, we will show that if $C(\Phi)^{\epsilon'}$ is approachable, then $\Phi \in \cS^{\epsilon}$. For the purposes of this section of the proof, we will assume that $C(\Phi)^{\epsilon'}$ is approachable. Now, consider a new polytope $M$, defined as follows: 
\[ M := \left\{ \phi \in \Delta^{mn} | u_{O,i}(\phi) \le u_{O,i}(\Phi_i) + \frac{B\epsilon}{k}, \forall i \in [k] \right\}\]

We will prove that $C(\Phi)^{\epsilon'} \subseteq M$.  To see this, consider any CSP $\phi^{*}$ in $C(\Phi)^{\epsilon'}$. Then, we have that 
$$\inf_{\phi \in C(\Phi)}||\phi^{*} - \phi||_{2} \leq \epsilon'$$

Because $C(\Phi)$ is a polytope and therefore closed, we can consider some $\phi^{**} \in C(\Phi)$ such that $||\phi^{*} - \phi^{**}||_{2} \leq \epsilon'$. We therefore have that  

$$ u_{O,i}(\phi^{**}) \le u_{O,i}(\Phi_i), \forall i \in [k]$$

And therefore that, for all $i$, 
\begin{align*}
  & ||\phi^{*} - \phi^{**}||_{2} \leq \epsilon' = \frac{B\epsilon}{k\sqrt{mn}}  \\
  & \implies u_{O,i}(\phi^{*}) - u_{O,i}(\phi^{**}) \leq \frac{B \epsilon}{k} \tag{By Cauchy-Schwartz and the fact that $u_{O,i} \in [-1,1]$}  \\
& \implies u_{O,i}(\phi^{*}) \leq u_{O,i}(\Phi_i) +  \frac{B\epsilon}{k}  \tag{By the fact that $u_{O,i}(\phi^{**}) \le u_{O,i}(\Phi_i), \forall i \in [k]$}  
\\ & \implies \phi^{*} \in M
\end{align*}

We have shown that $C(\Phi)^{\epsilon'} \subseteq M$. Therefore, by the upwards-closedness of menus shown in Corollary~\ref{corollary:upwards_closed}, since $C(\Phi)^{\epsilon'}$ is approachable, then $M$ is approachable. Now, let us consider $M'$, a subset of $M$, defined as follows:
\[ M' := \left \{ \phi \in \Delta^{mn} | u_{O,i}(\phi) \le \min(u_{O,i}(\Phi_i) + \frac{B\epsilon}{k}, L+_{i}), \forall i \in [k] \right\}\]

As $M$ is approachable, let $\cA$ be the algorithm which runs Blackwell approachability on the set $M$. Note that regardless of what the optimizer plays, it is not possible to obtain points $\phi$ such that $u_{O,i}(\phi) > L+_{i}$. Therefore, the menu of $\cA$ must be strictly contained within $M'$. Thus, $M'$ is also approachable.

Now, consider the k-CSP $\Phi^{*}$ which strictly increases the utility of every agent by $\frac{B \epsilon}{k}$ in the following way: let $i(1),...,i(mn)$ index the move pairs in increasing order of learner utility $i$. Then, we construct $\Phi^{*}$ as in Algorithm~\ref{alg:water}, which takes in a point $\Phi \in \cS^\varepsilon$ and outputs a $k$-CSP $\Phi^* \in \cS$.


\begin{algorithm}
    \begin{algorithmic}
     
    \FOR{$i \in [1,\ldots,k]$}
    \STATE $w \gets 0$ 
    \STATE $j \gets 1$
    \WHILE{$w < \frac{\epsilon}{k}$ \AND $j \leq mn$}
    \STATE $\Phi^{*}_{i}[i(j)] \gets \max(0, \Phi_{i}[i(j)] - \frac{\epsilon}{k} + w)$
    \STATE $w \gets w + \Phi_{i}[i(j)] - \Phi^{*}_{i}[i(j)] $
    \STATE $j \gets j+1$
    \ENDWHILE
    \STATE $\Phi^{*}_{i}[i(mn)] \gets \Phi_{i}[i(mn)] + w)$
    \ENDFOR
    \end{algorithmic}
    \caption{\label{alg:water}}
\end{algorithm}

Informally: for every $i$, for $\Phi_{i}$, we decrease the weight on the worst move pairs for agent $i$ (not going below zero) until the total weight has been decreased by $\frac{\epsilon}{k}$ or we run out of move pairs, and then we increase the weight on $L+_{i}$ by the total amount decreased. In doing this, for every $i$, there are two possibilities:
\begin{itemize}
    \item There is at least $\frac{\epsilon}{k}$ weight on action pairs in $\Phi$ that are not $L+_{i}$. Then, $u_{O,i}(\Phi_{i}^{*}) > u_{O,i}(\Phi_{i}) + \frac{B\epsilon}{k}$, where $B$ is the smallest gap between utilities in the game. 
    \item $\Phi_{i}^{*} = L+$. 
\end{itemize}

Thus, we have that for all $i$, $u_{O,i}(\Phi^{*}_{i}) \geq \min(u_{O,i}(\Phi_i) + \frac{B\epsilon}{k}, L+_{i})$. Therefore, $C(\Phi^{*}) \supseteq M'$, and since $M'$ is approachable, $C(\Phi^{*})$ is approachable. Therefore, $\Phi^{*} \in \cS$. 

Now, note that the $\ell_1$-distance between $\Phi^{*}$ and $\Phi$ is at most $k \cdot \frac{\epsilon}{k} = \epsilon$, by construction, and this upper bounds the $\ell_2$ distance. Furthermore, recall that $\Phi^{*} \in \cS$. Therefore, $\Phi \in \cS^{\epsilon}$. 



Finally, we must show that, if $C(\Phi)$ is not approachable, then $\Phi \notin \cS$. But this follows directly from the definition of $\cS$, so we are done.

Using the algorithm in Theorem~\ref{thm:tsitsiklis} with $\epsilon' = \frac{B\epsilon}{k\sqrt{mn}}$, the total runtime is 
\begin{align*}
  &   Poly(\frac{k}{\epsilon'})\cdot 2^{Poly(mn)} \\
  & = Poly(\frac{k^{2}\sqrt{mn}}{B \epsilon})\cdot 2^{Poly(mn)} \\
  & = Poly(\frac{k}{B \epsilon}) \cdot 2^{Poly(mn)}
\end{align*}




\end{proof}

\begin{theorem}
\label{thm:approachability_oracle2}
    There is an algorithm with running time $ \text{Poly}(\frac{mn}{\varepsilon}) \cdot 2^{\text{Poly} (k)}$ that is a $\varepsilon$-membership oracle for the set $\cS$. 
\end{theorem}
\begin{proof}
    The algorithm operates as follows: given some k-CSP $\Phi$, compute the result of \ref{thm:tsitsiklis} for the set $\cC_{v}(\Phi)$ on the Menu approachability game defined in Definition~\ref{def:menu_game_u} using the approximation parameter of $\epsilon' = \frac{\epsilon}{mn\sqrt{k}}$. This will reveal either that $\cC_{v}(\Phi)^{\epsilon'}$ is approachable, or $\cC_{v}(\Phi)$ is not approachable. In the first case, our algorithm outputs that $\Phi \in \cS^{\epsilon}$. in the second case, our algorithm outputs that $\Phi \notin \cS$. \nat{working here}
\end{proof}

\begin{corollary}
    There is an algorithm 
\end{corollary}

\begin{lemma}
    \label{lemma:ic_membership}
    There is a polynomial time membership oracle for the set $\cR$.
\end{lemma}

\begin{lemma}
%\label{corollary:intersection_membership}
    There is an algorithm with running time $\min \left\{ \text{Poly}(\frac{mn}{\varepsilon}) \cdot 2^{\text{Poly}(k)}, \text{Poly}(\frac{k}{\varepsilon}) \cdot 2^{\text{Poly} (mn)}\right\}$ that is a $\varepsilon$-membership oracle for the (convex) set $\cR^\varepsilon \cap \cS^\varepsilon$.
\end{lemma}



\subsection{Proof of Theorem~\ref{thm:main_result_without_nr}}

\begin{algorithm}
\caption{DistOpt} \label{alg:d-opt-2}
    \begin{algorithmic}
     \STATE Input: A learner utility $u_{L}$ and a distribution over optimizer utilities $\mathcal{D}$. \STATE Employ the membership oracle in Corollary~\ref{corollary:intersection_membership} and a standard algorithm to optimize a linear function in a convex set (see~\cite{grotschel2012geometric}) in order to attain $x \in \cR^\varepsilon \cap \cS^\varepsilon$ such that $V_L(x) \ge \max_{y \in \cR^\varepsilon \cap \cS^\varepsilon} V_L(y) - \delta$.
     \STATE Find a point $s \in \cS$ such that $d(x,s) \le \varepsilon$.
     \STATE Construct the set $\cM : = \text{Conv} \{\cC(s) \cup \{\phi_1,\phi_2 \cdots \phi_k\} \}$.
    \end{algorithmic}
\end{algorithm}

\begin{proof}
Employing the membership oracle in Corollary~\ref{corollary:intersection_membership} and a standard algorithm to optimize a linear function in a convex set (see~\cite{grotschel2012geometric}) gives us $x \in \cR^\varepsilon \cap \cS^\varepsilon$ such that $V_L(x) \ge \max_{y \in \cR^\varepsilon \cap \cS^\varepsilon} V_L(y) - \delta$. The running time of this algorithm is $\log{\left(\frac{1}{\delta} \right)} \cdot \min \left\{ \text{Poly}(\frac{mn}{\varepsilon}) \cdot 2^{\text{Poly}(k)}, \text{Poly}(\frac{k}{\varepsilon}) \cdot 2^{\text{Poly} (mn)}\right\}$. Since $\cP \subseteq \cR^\varepsilon \cap \cS^\varepsilon$, Lemma~\ref{lemma:wlog_polytope} implies that $V^* \le \max_{y \in \cR^\varepsilon \cap \cS^\varepsilon} V_L(y)$, implying that $V_L(x) \ge V^* -\delta$.
    \item Since $x \in \cR^\varepsilon \cap \cS^\varepsilon$, there exist points $ r \in \cR$ and $s \in \cS$ such that $d(x,r) \le \varepsilon$ and $d(x,s) \le \varepsilon$. The triangle inequality gives $d(r,s) \le 2 \varepsilon$. Since all the payoff vectors are within the bounds $[-1,1]^{mn}$, $V_L(s) \ge V_L(x) -2\varepsilon \ge V^* - (2\varepsilon+\delta)$.
    \item Write $s  = (\phi_1, \phi_2 \cdots \phi_k)$ and $r  = (\phi'_1, \phi'_2 \cdots \phi'_k)$. Since $d(r,s) \le 2 \varepsilon$, $u_{O,i}(\phi_i) \ge u_{O,i}(\phi'_i) -  2 \varepsilon$ and $u_{O,i}(\phi_j) \le u_{O,i}(\phi'_j) +  2 \varepsilon$ for all $i,j \in [k]$. However, since $r \in \cR$, $u_{O,i}(\phi'_i) \ge u_{O,i}(\phi'_j)$, thus we get $u_{O,i}(\phi_i) \ge u_{O,i}(\phi_j) - 4 \varepsilon$ for all $i,j \in [k]$ ,i.e., the incentive compatibility constraints are approximately satisfied by the point $s$. Construct the set $\cM : = \text{Conv} \{\cC(s) \cup \{\phi_1,\phi_2 \cdots \phi_k\} \}$. First, we see that $\cM$ is a feasible menu, since $\cC(s)$ is a feasible menu (due to $s \in \cS$) and menus are upwards closed~\ref{corollary:upwards_closed}. Second, we see that $u_{O,i}(\phi_i) \ge u_{O,i}(\phi) - 4 \varepsilon$ for all $\phi \in \cM$ (using the properties of $\cC$ and the inequalities proved in the last step). If the optimizer type is willing to take a hit of up to $4 \varepsilon$ while best-responding in the menu $\cM$, the point $p_i$ picked by the $i$-th optimizer satisfies $u_L(p_i) \ge u_L(\phi_i)$ since we have just shown that $\phi_i$ is a candidate point for the $i$-th optimizer type.
    
    Thus, $V^{4 \varepsilon}_L(\cM) \ge V_L(S) \ge V^* - (2 \varepsilon + \delta)$, completing the proof of Theorem~\ref{thm:main_result_without_nr}.    
\end{proof}




\subsection{Hardness of Menu Testing}

\begin{theorem}[Informal]

Testing if the polytope induced by a $k$-CSP is  NP-hard.
    
\end{theorem}

We outline the intuition behind the proof of this theorem --

\begin{itemize}
    \item ~\cite{mannor2009approachability} show that testing the approachability of a given set is NP-hard via a reduction from 3-SAT. In fact, they show something even stronger, which is that testing if the positive orthant is an approachable set for a given multivalued game and a set of optimizer payoffs is NP-hard.
    \item We reduce the latter problem to that of testing if the polytope induced by a $k$-CSP.
    \item The idea behind this reduction is that the polytope induced by a $k$-CSP in type space (dimension $k$ - defining a vector valued game that records all optimizer type payoffs) is the set of all points (i.e. $k$ payoffs) of realizable value that are pareto-dominated in this space by the optimizer values associated with the $k$-CSP. 
    \item We can add all points that are pareto-dominated WLOG since the extra points are not realizable and do not decide approachability/ exlcudability.
    \item Further, we can translate the payoff vector over all optimizers associated with the $k$-CSP to be the origin WLOG. Further, we can reverse the signs to flip the non-positive and the non-negative orthant, completing the reduction.
\end{itemize}




==> includes2.tex <==
\usepackage[utf8]{inputenc}
\usepackage[numbers]{natbib}
\usepackage{amsmath,amssymb}
\usepackage{bbm}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
%\usepackage{algpseudocode}
%\usepackage[ruled]{algorithm2e}
 \usepackage{algorithm}
 \usepackage{algorithmic}
%\usepackage[]{algorithm2e}
%\RestyleAlgo{boxruled}
 
%\usepackage[usenames,dvipsnames]{xcolor}

%\usepackage{tcolorbox}
%\tcbuselibrary{skins,breakable}
%\tcbset{enhanced jigsaw}


%\colorlet{YellowOrange}{RawSienna}
%\newcommand{\nat}[1]{\textcolor{blue}{[Natalie: #1]}}
%\newcommand\jon[1]{{[\color{magenta}{\textbf{Jon:}~#1}]}}
\newenvironment{proofof}[1]{\par{\noindent \bf Proof of #1:}}{$\blacksquare$ \par}
\newenvironment{oneshot}[1]{\@begintheorem{#1}{\unskip}}{\@endtheorem}
\usepackage{hyperref}
%\hypersetup{
%colorlinks=true,
%pdfnewwindow=true,
%citecolor=ForestGreen,
%linkcolor=DarkRed,
%filecolor=DarkRed,
%urlcolor=DarkBlue
%}
\usepackage{cleveref}

\newcommand{\tempcol}[1]{{\color{red}#1}}

\usepackage{fullpage}
\newtheorem{observation}[theorem]{Observation}
%\usepackage[pdftex]{graphicx}

%\usepackage{xcolor}
%\newcommand{\esh}[1]{\textcolor{red}{[Eshwar: #1]}}
%\newcommand{\sk}[1]{\textcolor{blue}{[Sampath: #1]}}
%\newcommand{\ad}[1]{\textcolor{green}{[Anindya: #1]}}
\newcommand{\ade}[1]{\textcolor{red}{#1}}
\newcommand{\hdn}{homogeneous noise model}



\newcommand{\expect}[1]{\mathbb{E}\left[#1\right]}

\usepackage{comment}
\usepackage{mathtools}

\usepackage[shortlabels]{enumitem}


\newcommand{\X}{\mathcal{X}}
\newcommand{\sst}{\text{special subtree}}
\newcommand{\fs}{\sqrt{\frac{\log n}{n}}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Mh}{\mathbf{Q}_h}

\usepackage[shortlabels]{enumitem}

\newcommand{\ignore}[1]{}
\newcommand{\fsi}{\sqrt{\frac{n}{\log n}}}
\newcommand{\ohp}{overwhelmingly high probability}
\newcommand{\hide}[1]{}


%New Commands from Edited Weights

\usepackage[shortlabels]{enumitem}
\newcommand{\NL}{\mathsf{NL}}
\newcommand{\lc}{\mathsf{lc}}
\newcommand{\rc}{\mathsf{rc}}
\newcommand{\bebetter}{b_{\text{better}}}
%\newcommand{\coloneqq}{:=}



\usepackage[shortlabels]{enumitem}

\newcommand{\p}{\widetilde{p}}
\newcommand{\h}{\widehat{h}}


\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}

\newcommand{\M}{\mathcal{M}}

\usepackage{caption}
\usepackage{xcolor}

\newcommand{\brmix}{S'}

% jon commands


\def\Rset{\mathbb{R}}
\def\Sset{\mathbb{S}}

\let\Pr\undefined
\let\P\undefined
\DeclareMathOperator*{\Pr}{\mathbb{P}}
\DeclareMathOperator*{\P}{\mathbb{P}}
% \DeclareMathOperator*{\E}{\mathbb E}
% \DeclareMathOperator*{\argmax}{argmax}
% \DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\esssup}{esssup}
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\cont}{cont}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\core}{core}
\DeclareMathOperator*{\pen}{pen}
\DeclareMathOperator{\VCdim}{VCdim}
\DeclareMathOperator{\Pdim}{Pdim}
\DeclareMathOperator{\Reg}{\mathsf{Reg}}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\diag}{diag}


\DeclareMathOperator{\Ind}{\mathbb{I}} 

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert} 
\DeclarePairedDelimiter{\bracket}{[}{]}
\DeclarePairedDelimiter{\curl}{\{}{\}}
\DeclarePairedDelimiter{\norm}{\|}{\|}
\DeclarePairedDelimiter{\paren}{(}{)}
\DeclarePairedDelimiter{\tri}{\langle}{\rangle}
\DeclarePairedDelimiter{\dtri}{\llangle}{\rrangle}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\sA}{{\mathscr A}}
\newcommand{\sB}{{\mathscr B}}
\newcommand{\sC}{{\mathscr C}}
\newcommand{\sD}{{\mathscr D}}
\newcommand{\sF}{{\mathscr F}}
\newcommand{\sG}{{\mathscr G}}
\newcommand{\sH}{{\mathscr H}}
\newcommand{\sI}{{\mathscr I}}
\newcommand{\sJ}{{\mathscr J}}
\newcommand{\sK}{{\mathscr K}}
\newcommand{\sL}{{\mathscr L}}
\newcommand{\sM}{{\mathscr M}}
\newcommand{\sP}{{\mathscr P}}
\newcommand{\sS}{{\mathscr S}}
\newcommand{\sT}{{\mathscr T}}
\newcommand{\sU}{{\mathscr U}}
\newcommand{\sX}{{\mathscr X}}
\newcommand{\sY}{{\mathscr Y}}
\newcommand{\sZ}{{\mathscr Z}}

\newcommand{\bA}{{\mathbf A}}
\newcommand{\bB}{{\mathbf B}}
\newcommand{\bD}{{\mathbf D}}
\newcommand{\bH}{{\mathbf H}}
\newcommand{\bK}{{\mathbf K}}
\newcommand{\bL}{{\mathbf L}}
\newcommand{\bM}{{\mathbf M}}
\newcommand{\bN}{{\mathbf N}}
\newcommand{\bP}{{\mathbf P}}
\newcommand{\bQ}{{\mathbf Q}}
\newcommand{\bR}{{\mathbf R}}
\newcommand{\bV}{{\mathbf V}}
\newcommand{\bW}{{\mathbf W}}
\newcommand{\bX}{{\mathbf X}}
\newcommand{\bY}{{\mathbf Y}}
\newcommand{\bZ}{{\mathbf Z}}
\newcommand{\bb}{{\mathbf b}}
\newcommand{\bl}{{\mathbf l}}
\newcommand{\bx}{{\mathbf x}}
\newcommand{\by}{{\mathbf y}}
\newcommand{\bu}{{\mathbf u}}
\newcommand{\bv}{{\mathbf v}}
\newcommand{\bw}{{\mathbf w}}
\newcommand{\bp}{{\mathbf p}}
\newcommand{\bell}{{\bm \ell}}

\newcommand{\sfp}{{\mathsf p}}
\newcommand{\sfq}{{\mathsf q}}
\newcommand{\sfr}{{\mathsf r}}
\newcommand{\sfE}{{\mathsf E}}
\newcommand{\sfB}{{\mathsf B}}
\newcommand{\sfD}{{\mathsf D}}
\newcommand{\sfS}{{\mathsf S}}
\newcommand{\sfT}{{\mathsf T}}

\newcommand{\eps}{{\varepsilon}}


\DeclareMathOperator{\Prof}{\mathsf{Prof}}
\newcommand{\MB}{\M_{\mathrm{MB}}}
\DeclareMathOperator{\BR}{\mathsf{BR}}


%Macros

\newcommand{\csp}{\varphi}
\newcommand{\gameset}{\mathcal{G}}
\newcommand{\Up}{U^{+}}
\newcommand{\Um}{U^{-}}
\newcommand{\Mp}{\M^{+}}
\newcommand{\Mm}{\M^{-}}
\newcommand{\Uzs}{U_{ZS}}
\newcommand{\ox}{\overline{x}}


\newcommand{\boundary}{T^{1-\tau}}
\newcommand{\regret}{\alpha}


\newcommand{\intersectionmb}{\mathcal{M}_{MI}}


\newcommand{\ftraj}{finite trajectory}

\newcommand{\ftrajs}{finite trajectories}




%The comment commands and their alternate forms
\newcommand{\esh}[1]{\textcolor{red}{[Eshwar: #1]}}
%\newcommand{\esh}[1]{}

\newcommand{\nat}[1]{\textcolor{blue}{[Natalie: #1]}}
%\newcommand{\nat}[1]{}
\newcommand\jon[1]{{[\color{magenta}{\textbf{Jon:}~#1}]}}
%\newcommand\jon[1]{}


%Macros for notation

\newcommand{\optdist}{\mathcal{D}}

\newcommand{\algfams}{\mathcal{F}_\mathcal{A}}
\newcommand{\nralgs}{\mathcal{F}_\mathcal{NR}}



%New macros for EC submission, copy into the other includes fule
% \newcommand{\ftrl}{\textsf{FTRL-fixed-convex}}
\newcommand{\ftrl}{\textsf{FTRL}}
\DeclareMathOperator{\regbound}{\rho}
\newcommand{\wtA}{\widetilde{A}}
\newcommand{\opt}{\text{opt}}
\DeclareMathOperator{\sshift}{\zeta}
\usepackage{nicematrix}
